Thermal Dissipation Resulting from Everyday Interactions as a Sensing Modality -- The MIDAS Touch

We contribute MIDAS as a novel sensing solution for characterizing everyday objects using thermal dissipation. MIDAS takes advantage of the fact that anytime a person touches an object it results in heat transfer. By capturing and modeling the dissipation of the transferred heat, e.g., through the decrease in the captured thermal radiation, MIDAS can characterize the object and determine its material. We validate MIDAS through extensive empirical benchmarks and demonstrate that MIDAS offers an innovative sensing modality that can recognize a wide range of materials with up to 83% accuracy and generalize to variations in the people interacting with objects. We also demonstrate that MIDAS can detect thermal dissipation through objects, up to 2 mm thickness, and support analysis of multiple objects that are interacted with

==> The MIDAS Touch1/sections/Abstract.tex <==

We contribute \SystemName{} as a novel sensing solution for characterizing everyday objects using thermal dissipation. \SystemName{} takes advantage of the fact that anytime a person touches an object it results in heat transfer. %that can be captured. %by a thermal camera.
By capturing and modeling the dissipation of the transferred heat, e.g., through the decrease in the captured thermal radiation, \SystemName{} can characterize the object and determine its material. We validate \SystemName{} through extensive empirical benchmarks and demonstrate that \SystemName{} offers an innovative sensing modality that can recognize a wide range of materials -- with up to $83\%$ accuracy -- and generalize to variations in the people interacting with objects. We also demonstrate that \SystemName{} can detect thermal dissipation through objects, up to \SI{2}{mm} thickness, and support analysis of multiple objects that are interacted with. 



==> The MIDAS Touch1/sections/Background.tex <==
\section{Background of study}
This section introduces public littering, which is considered a problem that plagues our society and the world. We also present background knowledge of the detection sensors, focusing on the thermal sensing technique and how it has been applied in computer systems. This technique is widely used in various fields of study. The thermal sensor can be integrated into an automated system such as autonomous robots or drones to detect common waste materials disposed on the streets, public areas, locate the material, and properly recycling it.  

\bparagraph{Public littering} Disposing of visible solid waste in wrong places or places they do not belong is considered as littering \cite{schultz2013littering}, \cite{campbell2007people}. It portrays a bad picture of the area, pollutes the environment, and costs a lot to clean up if not properly managed. Litter is distinct from other municipal solid waste (MSW) and includes any solid or liquid domestic debris. The most littered items are cigarette butts, takeout boxes, food wrappers, drink bottles or cans, broken glass, plastic bags. In 2007, the international coastal cleanup, Ocean Conservancy collected 6 million pounds of materials, which comprised of cigarette butts (27\% of the total number of items collected), bags(8\%), plastic beverage bottles (7\%), plastic utensils (5\%), caps and lids (9\%), and food wrappers (10\%) \cite{conservancy2007start}. Research has shown people's behavioural tendencies towards littering; there is a correlation between a littered environment and the intentional throwing of litter at that particular spot littered \cite{finnie1973field}. This means that when a place is littered, there is a higher propensity to experience increased littering. Littering is attributed to individuals as the primary source \cite{schultz2013littering}. 

Furthermore, it is estimated that 4.95 trillion cigarette butts are littered yearly worldwide, which also presents a threat to wildlife and, in some cases, fire outbreaks \cite{world2017tobacco}. Cigarette filters have been discovered in the stomachs of sea or marine creatures, birds who mistake them for food \cite{santos2005overseas}. Globally, different approaches have been adopted to curb littering to slow down climate change, such as providing the convenience of disposal facilities, public awareness on environmental education by promoting a positive attitude towards the environment, enforcement by handing out fines to perpetrators. There is no doubt that people have heard a lot about environmental problems, and they now want to hear a lot more about environmental solutions. 


\bparagraph{Passive sensing (IR Thermal imaging)}
According to J. Fraden,  “A sensor is a device that receives stimulus or an input signal and responds with an electrical signal bearing a known relationship to the input” \cite{fraden2003handbook}. Sensors can be found in most electrical devices and are designed for various applications, as well as aids surveillance, imaging, tracking, detecting, and mapping. Two categories of sensors consist of active sensor, which provides their source of light or illumination while also transmitting and detecting energy simultaneously. On the other hand, passive sensors do not provide illumination to produce output signals and measure variations based on natural emission \cite{brooker2009introduction}.

Infrared Thermal imaging, also known as Infrared thermography, is the recording and measurement of heat radiation. These are specially-designed cameras that work in an environment without any ambient light and can penetrate obscurants such as smoke, fog, and haze. The first Thermal cameras were originally developed for military purposes in 1950s and 1960s and have since evolved, enabling applications that were impossible to do easily in the past due to the high cost of production and limited availability. Thermal cameras are similar to digital photographic cameras but record thermal infrared radiation (TIR). Infrared radiation is invisible to the human eye as it occurs beyond the red end of the visible light spectrum (figure 1). However, thermal radiation is located within the infrared range of the electromagnetic spectrum \cite{kruse2001uncooled}. The visible wavelength range from $0.4 - 0.78\mu m$ while infrared radiation has a longer wavelength, ranging from $0.78-1000\mu m$ \cite{mehta2011introduction}; Thermal cameras operate in the infrared band of the electromagnetic spectrum with wavelengths between $2 - 14\mu m$. The infrared spectrum which is subdivided into near-infrared (NIR) $0.78 - 2.5\mu m$, mid-infrared (MIR) $1.3 - 8\mu m$ and far-infrared (FIR) $7.5\mu m$ and $13\mu m$ \cite{abdelrahman2017cognitive}, and are used for monitoring temperatures of different range from -50 to 2000$^{\circ}$C. All objects with a temperature above absolute zero (-273$^{\circ}$C) emit infrared radiation and not only objects we think of as warm emit infrared radiation (IR). Thermal imaging determines an image temperature based on the absolute temperature of the object. The image is formed base on the heat signature of the object and records current signatures of the objects based on their heat pattern.


%\begin{figure}
%	\centering
%		\includegraphics[width=0.4\textwidth]{graphics/spec.png}
%	\caption{The electromagnetic spectrum\cite{vadivambal2011applications}}
%	\label{fig:EngProto}
%\end{figure}

\subsection{Thermal detection types}
Thermal detection mechanism referred to as mechanism that change some measurable property of a material due to the temperature rise of that material caused by the absorption of electromagnetic radiation \cite{lloyd2013thermal}. Although there are several thermal detection mechanism, the most important are the resistive bolometric effect,  the pyroelectric effect and its modification known as either the biasenhanced pyroelectric effect or the ferroelectric bolometer, and the thermoelectric effect \cite{lloyd2013thermal}. Uncooled thermal detectors have been developed mainly with microbolometers thermal and ferroelectric detectors (uses Barium strontium titanate (BST) as detector material, which suffers from halo effect) \cite{gade2014thermal}. Microbolometers has the largest market share due to its advantages over ferroelectric detectors. 


\subsection{Application in computer systems}
With thermal imaging becoming popular, this section briefly discuses thermography as a useful technology in different fields. This detection technique is used in computer systems, which uses sophisticated image analysis algorithms and a computer to reconstruct the images to show heat patterns.

\bparagraph{Medical thermography} Computer systems are used for image processing and monitoring of thermal radiation changes. In medical analysis, thermography based computer-assisted detection/diagnosis (CAD) systems help to screen for fever patients in places with a high volume of people, such as airports and border crossings \cite{mercer2009fever}, \cite{sun2011portable}. The early detection of the diabetic foot,  specifically, CAD systems for diabetic foot \cite{adam2017computer}, help prevent complications and amputation. They have also been shown to reveal tumors in an early stage, most notably breast cancer \cite{qi2003thermal}. Medical issues such as the behaviour of ciliary muscle of the human eye \cite{harangi2011detecting}, the periodic fluctuation in skin temperature \cite{kondo2001thermal} or the measuring of blood flow rate in superficial veins \cite{mahmoud2013non}, can be studied from thermal images.

\bparagraph{Facial analysis} The face of an individual is a biometric trait that can be applied in an automated computer-based security system for authentication purposes. Experts are investigating and developing methods for the improvement of face recognition \cite{bhowmik2008classification}. Humans' stress level can be detected using thermal imaging, based on the heat radiation from their face. Thermal facial analysis was used for deception detection \cite{rajoub2014thermal}. Pavlidis et al. \cite{pavlidis2006detection} also propose this technique to capture anxiety. 

\bparagraph{Fire detection and military} With firefighters' inability to see through smoke quickly, they can be robbed of their most essential commodities (sight) when they fight fires and as such handicapping their ability to perform effectively, find the hot spot, and locate victims. Identification of objects that could pose a risk is of great importance. A fire detection system can be used for mobile robots \cite{hwang2010novel} by locating the hot spots, the robot is directed to the fire source. Arrue et al. \cite{arrue2000intelligent} proposed an alternative real-time infrared-visual system for forest fire detection, composed of both thermal and visual cameras, and meteorological and geographical information. In the military, Price et al. \cite{price2004system} presented the Gunfire Detection and Location (GDL) system for military applications to detect gunfire. Gunfire is detected in Mid-Wave IR (MWIR) imager and validated by acoustic events.










==> The MIDAS Touch1/sections/Conclusions.tex <==
\section{Summary and Conclusions}

%that uses human-emitted thermal radiation to classify different material waste types. \

We developed \SystemName{} as an innovative sensing solution for characterizing and recognizing everyday objects from the dissipation of residual thermal energy resulting from human touch. \SystemName{} uses thermal imaging to monitor thermal energy changes over time and models these changes to infer and characterize the material type of an object. Through extensive empirical benchmarks, we demonstrated that changes in thermal fingerprints are robust to variations in the way people interact with objects and the people themselves. \SystemName{} recognizes different material with up to $83\%$ accuracy using only the dissipation of thermal fingerprints. Our solution offers an innovative sensing solution for classifying materials and taking advantage of human interactions with everyday objects.



==> The MIDAS Touch1/sections/Discussion.tex <==
\section{Discussion}
\label{sec:Discussion}

\cparagraph{Human temperature} Human temperature changes in cycles, being at its highest during hours of activity (day) and lowest during sleep (night)~\cite{obermeyer2017individual}. We demonstrate that interactions with objects can be used to characterize materials. The best results are obtained when the body temperature is stable, but the relative differences in thermal fingerprints are consistent across variations in body temperature. Conversely, interactions with an object of known material and in a stable environment can be used to detect relative differences in body temperature.

%such temperature measured during day hours can be used to characterize object  materials. 

\cparagraph{Room for improvement} \rev{Naturally, there are further challenges that need to be addressed to make our solution more robust across diverse environments.} Adapting our approach to continuous monitoring requires accurate and noise-free thermal images, e.g., using calibration~\cite{malmivirta2019hot}. Not all materials can be characterized using our solution as thermal cameras have different emissivity ranges and some materials may reflect too much -- or too little -- thermal radiation. Such materials are usually used to preserve user's privacy, e.g., ATM pin codes~\cite{abdelrahman2017stay}. The experiments were conducted using thermal cameras integrated into smartphones, but in the future it may be possible to use cheaper alternatives, such as low-cost thermal array sensors~\cite{rintahomi21how}. \rev{There are also challenges arising from practical deployments as environments with oscillating temperatures can result in unstable fingerprints and as there can be situations where only partial dissipation fingerprints are available (e.g., due to the use of gloves).}  While outside the scope of our present work, there is also room for developing application areas, e.g., validating temperature differences with patients as part of clinical studies.  % However, we need access to clinical experts and additional permissions from our University ethics department to do this.

 %For example, fast oscillations in ambient temperature can affect the characteristics of thermal dissipation fingerprints and degrade the performance of our technique. These cases can be overcome using contextual profiles and additional information to select the best suited profile.
%Similarly, contexts where there thermal dissipation is partial can cause difficulties, e.g., if the person is wearing gloves or there is no sunlight or other source of thermal radiation. 

\cparagraph{Other material properties} Dissipation time of thermal fingerprint gives insights about material types and correlates with emissivity. Thermal imaging could be used to potentially infer other material properties, such as thickness and elasticity. Potential use cases include detecting the pollutant type of marine plastics~\cite{flores2021toward} and monitoring the decay in organic materials using differences in thermal dissipation characteristics. %, thermal radiation is spread and absorbed on the surface based on material type. We are interested in exploring those and organic materials, which are prone to decay and visual changes. 

\cparagraph{Micro-expressions through hand-touch} Micro-expressions are facial expressions captured in a fraction of time by cameras. Our work demonstrates that the thermal fingerprint of a hand-touch on an object has a life span that depends on how long the object was held. Thus, thermal analysis of human touch can be another approach for detecting micro-expressions, e.g., disgust and excitement. Similarly, micro-expressions through human-touch can be envisioned as an approach to measuring individuals' productivity at work. 

\cparagraph{Robots and autonomous devices} Thermal radiation analysis of objects touched by humans can be used to inform and train different robots and autonomous devices, e.g., UAVs~\cite{liyanage2021geese}, about the material properties of objects. New sensing and interaction modalities can also be envisioned as part of robotic systems, e.g., incorporating heat sensation to detect the material of an object and to enable autonomous devices to adjust their operations with objects in the surrounding environment~\cite{li2020skin}. For instance, a robotic arm can rely on a camera to detect an empty bottle on a table. However,  the arm's pressure to lift and put the bottle should be proportional to the bottle material. Otherwise, the robotic arm can break apart the bottle, e.g., plastic vs. glass bottle. Besides, since it is possible to differentiate thermal radiation emitted by different genders, autonomous devices can adjust their interactions accordingly. 

%\cparagraph{Practical Integration} As part of the experiments we demonstrated that \SystemName{} can operate through objects, up to approximately \SI{2}{mm} thickness depending on the material of the object. This offers potential for integrating \SystemName{} inside objects or under objects that are being interacted with. As an example, intelligent surfaces could measure dissipation patterns of objects that are placed on the surface, and toys~\cite{fan2014injecting} and other smart objects could integrate thermal cameras inside them to offer new types of personalized interactions.

\cparagraph{Augmented Reality systems} Augmented Reality systems that mix the real and virtual worlds can benefit from thermal radiation monitoring. By piggybacking the human-touch on objects, it is possible to recognize the materials of objects further. These objects are mapped to the virtual world by considering their inherent natural material properties, such as wood, concrete, glass, and plastic.

%potentially to be removed
%\cparagraph{Other pervasive systems} Several other pervasive systems can benefit from our thermal approach. Health monitoring systems can track temperature from individuals while preserving their privacy by monitoring objects' thermal fingerprints instead of direct human measurements are taken from different body parts, e.g., forehead and hands. Similarly, new sensing modalities that pre-warm the materials to understand the composition in different environments can be envisioned, e.g., cold and underwater environments. 

%This type of sensing scenario is highly relevant for emerging IoT scenarios, where sensors capture interactions from users not from the outer side of the object's surface but rather from its inner side. In other words, sensors monitor the external interactions of users from the inside of the object. For example, near-infrared and USB thermal cameras are small enough to be embedded anywhere to support diverse use cases, e.g., elderly medication management or toys embedding sensors


\cparagraph{Application scenarios} \rev{The core focus of our work has been on showing the potential of using thermal dissipation as a sensing modality without focusing on any specific application scenario. Nevertheless, thermal dissipation has significant potential for many real-world application scenarios. One application area is household waste sorting as humans interact with waste objects just before they are thrown to the bin. Our approach allows using the residual thermal energy resulting from these interactions to identify which type of material the object consists of and to support better recycling practices. In our ongoing work, we have also shown how thermal dissipation resulting from sunlight can be integrated with autonomous ground vehicles (AGVs) to classify litter thrown on the ground~\cite{yin2022toward}. Our results also showed that thermal dissipation can be sensed from the inside of an object and this could be used as an alternative to identify interactions. For example, an interactive toy could detect when a child plays with it~\cite{fan2014injecting}. Another interesting application would be to integrate the sensors as part of medical bottles to support medication management~\cite{klakegg2018assisted}. Exploring these opportunities is an interesting venue for future research. Naturally, realising these scenarios requires further advances in thermal sensing technology. Firstly,  miniaturization of thermal cameras is required. While currently USB size solutions are available, they generally expect a sufficient power source and processing unit (e.g., a smartphone). It is expected further miniaturization of the technology as the one achieved by existing RGB-camera, e.g., pen-size cameras. Secondly, thermal dissipation time also needs to be characterized for this purpose. Indeed, in our experiments, we demonstrate that while thermal dissipation time can be measured from both sides of the object (inner and outer sides), both thermal dissipation differed as a result of thermal loss. Thus, thermal dissipation time has to be pre-computed considering different thicknesses. }




==> The MIDAS Touch1/sections/ExperimentalSetup.tex <==
\section{Robustness of Thermal Dissipation Fingerprints } 
\label{sec:experimentalsetup}


The experiments shown in Sec.~\ref{sec:materialselection} demonstrated that the dissipation characteristics of thermal fingerprints vary across different materials. Human body temperature varies across individuals and even within the same individual at different times of day~\cite{obermeyer2017individual}, which results in variations in the initial thermal fingerprints. Ensuring \SystemName{} can operate robustly against these variations is essential for ensuring the usefulness of \SystemName{} in practical use. In this section, we describe experiments where $18$ different individuals touch everyday objects, and we use the resulting thermal fingerprints and their dissipation to characterize the materials of the objects. The measurement setup is described in Section~\ref{ssec:testbed}. \rev{The experiments rely on measurements captured in an experimental testbed designed to capture video footage of thermal fingerprints for different objects materials. For this purpose, we used an off-the-shelf smartphone thermal camera and a thermometer scanner to measure the reference baseline. We consider three different materials which were chosen to have different shapes and sizes, but also to have sufficiently fast dissipation time to reduce the overall length of the study.}



\subsection{Experimental Setup}



\cparagraph{Experiment Design} 

We conduct a $3\times3$ within-subject design with holding pattern type and object type as independent variables. Both variables have three levels: Fixed-hold (FH), Natural-hold (NH) and Quick-hold (QH) for the former and Plastic bottle (BOTTLE), Cardboard cup (CUP) and Cigarette butt (CIGAR) for the latter. To eliminate order effects, whilst keeping the number of combinations manageable, holding pattern type was fully counterbalanced, whereas object type was counterbalanced following a Latin Square design, resulting in %The experiment conditions were counterbalanced, resulting in 
nine experimental conditions: %Combining the three object types and the three levels of thermal radiation transferred resulted in nine experiment conditions:\ 
(1) BOTTLE-FH, (2) CUP-FH, (3) CIGAR-FH; (4) BOTTLE-NH, (5) CUP-NH, (6) CIGAR-NH; (7) BOTTLE-QH, (8) CUP-QH, and (9) CIGAR-QH. 
 

\begin{figure}[!t]
	\centering	\includegraphics[width=0.8\columnwidth]{graphics/fig4.png}
	\caption{Processing pipeline of material classification based on dissipation time of thermal fingerprints.}
	\label{fig:approach}
	   \vspace{-.4cm}
\end{figure}





In the~\textit{Fixed-hold} condition, objects were grabbed and held from a specific static position for one minute (Figure~\ref{fig:conditions}a). In the~\textit{Natural-hold} condition, objects were held freely for one minute, simulating usual everyday interactions with the object (Figure~\ref{fig:conditions}b). For instance, a participant holds the empty bottle for one minute while looking for a trash bin. In the~\textit{Quick-hold} condition, objects were held by participants freely for a \SI{10}{s} span.

%In total, our design includes $18$ participants $\times$ three thermal transferred conditions $\times$ three object materials = $146$ trials. 


\cparagraph{Participants} We recruited a total of N=$18$ participants (Males=$9$, Females=$9$) for the user study. Participants were students, admin staff and professionals from different fields, and nationalities, with little or no knowledge about thermal imaging. Their average age was $28\pm7.8$ years.% (SD$=7.8$).


\begin{figure}
	\centering
		\includegraphics[width=0.65\columnwidth]{graphics/fig5.png}
	\caption{Experimental conditions: (a) Rigid interaction, used in Fixed-hold and (b) Free interaction, used in Natural and Quick holds.}
	\label{fig:conditions}
\end{figure}




%\label{subsec:task}
\cparagraph{Task} 

Participants were asked to hold objects and to simulate normal interactions with them. To produce data for natural interaction, we also asked the participants to contextualize a normal interaction context. When interacting with the BOTTLE, participants were asked to simulate drinking from the bottle and then looking for a trash bin to dispose an empty bottle. Similarly, participants were asked to stand while engaging in a short conversation with an acquaintance/friend for the CUP. Finally, for the CIGAR condition, participants were asked to simulate taking a cigarette from a cigarette box and then holding the cigarette from the filter while asking for a light. The cigarette was not lighted during the experiment. 





\cparagraph{Procedure} Before starting the experiment, each participant was invited to relax on a comfortable chair for $10$ minutes to enable the body temperature to acclimatize to the room's ambient temperature, which oscillated around \SIrange{22}{23.5}{\degreeCelsius} %$22-23.5$\textcelsius~
throughout the experiments. During this period, participants received a brief explanation of the study and signed an informed consent form, following local IRB regulations. Once the participant was ready to start the experiment, his/her/their body temperature was measured from the forehead using a clinically certified contactless optical thermometer (DR CHECK FC500). The nine experimental conditions were presented to participants. 
In each condition, the object was first placed inside an empty fridge with a temperature of \SI{5}{\degreeCelsius} for one minute (Figure~\ref{fig:testbed}a). This procedure rules out residual thermal radiation in the material between experiments and provides the material with a baseline temperature to make our results comparable across the participants. % Researcher conducting the experiment used kitchen tongs to put in and take the object from the fridge, to avoid transferring his/her human thermal radiation. 

Kitchen tongs were used to take the object from the fridge to avoid heat transfer from humans to objects.
Next, the object was placed on a table for one minute to adapt it to the ambient temperature (Figure~\ref{fig:testbed}b). After that, participants carried out the corresponding experimental condition. Once finished, participants placed the object on a fixed marker drawn on a table with a black background and surface. The researcher conducting the study then used the CAT S60 to record video footage of the dissipation of the object's thermal fingerprint. In parallel, a thermometer scanner took thermal photos %during this time 
to serve as a reference baseline (Figure~\ref{fig:testbed}c). A black background helps to obtain clean video footage of thermal fingerprint without any thermal influence from objects in the surrounding environment. At the end of the experiment, we measured the participant's temperature from palm and finger to the objects using the thermal imaging scanner. The evaluation took place in one university room across two weeks in time slots between 11:00 and to 07:00 pm. % that fall within the interval of 11:00 am to 07:00 pm. 
Since human temperature varies during the day~\cite{obermeyer2017individual}, we considered only those times as they coincide with the working hours of the participants. For each participant, the overall experiment lasted  \SIrange{40}{45}{\minute}. 



\begin{figure}[!t]
	\centering
		\includegraphics[width=0.65\columnwidth]{graphics/fig6.png}
	\caption{Experimental testbed and protocol steps: (a) Object obtains baseline temperature, (b) Object habituates to ambient temperature, and (c) Participant performs the experiment and puts the object in the marked target to measure its thermal fingerprint.}
	\label{fig:testbed}
\end{figure}


 

\subsection{Baselines}

As part of the experiments, we compare the recognition performance of \SystemName{} to two state-of-the-art techniques: deep learning based automated computer vision~\cite{white2020wastenet,ruiz2019automatic} and optical sensing~\cite{singh2016iot}. 

\cparagraph{Computer Vision} We train a state-of-the-art Convolutional Neural Network (CNN) model using the publicly available TrashNet dataset~\cite{aral2018classification}. We focus exclusively on the plastic materials category, which contains $626$ images of plastic objects for training the deep learning model. Plastics are malleable, so their accurate recognition is very sensitive to changes. The dataset has images where the individual pieces are shown against a white background. As such images do not match realistic recognition settings. To overcome this, we supplement the dataset with an additional $767$ images from the Japan Agency for Marine Earth Science and Technology (JAMSTEC) Deep-sea Debris Database dataset. We annotated the collected images manually by drawing a rectangle box around the object material in images. We labeled the TrashNet plastic items as "trash" and the JAMSTEC plastic items as "plastic". Both datasets were augmented by adding noise, hue, blue, horizontal flip, and vertical flip modifications to each original image, resulting in a total of $6985$ images for model training input. We created and trained the PlasticNet model using Google Collab server GPU, performing 100k iterations with a batch size of 12, running TensorFlow Lite 1.15. We used~\textit{ssd\_mobilenetv2\_oidv4} for the base training model with default hyperparameters.

%Reflectivity analysis of materials is a highly adopted technique to classify different material types~\cite{singh2016iot}. 

\cparagraph{Light Reflectivity} As our second baseline, we consider reflectivity analysis of materials~\cite{singh2016iot} using a photoresistor connected to the analog input pin of an Arduino MEGA ADK. The photoresistor captures light changes based on its resistance exposure to the light intensity of the reflected material. As a light source, we rely on a red laser diode (wavelength \SI{650}{\nano\metre}). The object was located \SI{2}{\centi\metre} away from the light source, depicting a practical usage of the sensor in transport belts and smart bins~\cite{white2020wastenet}. We took measurements with sensor for different materials (selection is described in Section~\ref{sec:materialselection}), for one minute from two different random places in the object.





==> The MIDAS Touch1/sections/Introduction.tex <==
\section{Introduction}


Every day humans touch numerous objects, ranging from their personal possessions to home appliances, food, clothing, and many other objects~\cite{zuccotti2015every}. Capturing information about the objects people interact with has the potential to offer rich insights into human behaviour~\cite{klatzky1985identifying}. Such ranges from simple everyday activity monitoring to more complex applications, being dietary monitoring~\cite{bi2018auracle} or detection of household practices~\cite{babaei2015household}. Unfortunately, capturing such information is fraught with difficulty as current solutions suffer from some significant limitations. Specifically, contact-based approaches, such as RFID, either require instrumenting all objects or keeping the sensing device in close contact with the object for a sufficiently long period~\cite{ha2018learning, wang2017tagscan}. Non-contact based solutions, such as image-based object recognition, in turn, have limited discriminatory power and are sensitive to the conditions of the operating environment~\cite{yeo2017specam}.
% and are vulnerable to the environment where they are operated~\cite{yeo2017specam}.
For example, image-based recognition is prone to changes in illumination, camera angle, and picture resolution~\cite{schwartz2019recognizing}.

This paper develops \SystemName{} as a novel sensing solution for characterizing everyday objects using the thermal dissipation resulting from human touch. \SystemName{} exploits the fact that anytime a person touches an object it results in heat transfer. Over time, the transferred heat dissipates from the object as the object attempts to reach thermal equilibrium with the surrounding environment. The rate of this dissipation depends on the material characteristics of the object. \SystemName{} captures the heat transfer and the ensuing dissipation and uses these to model and characterize the materials of the objects that the user interacts with. \SystemName{} captures the changes in heat using a commercial-off-the-shelf (COTS) thermal camera. Thermal cameras can operate without requiring contact and they are robust to illumination conditions and the overall capture context, thus overcoming the key limitations of current techniques. Thermal imaging is also increasingly feasible thanks to the increase of thermal cameras in production. For example, several Caterpillar smartphones integrate forward looking infrared (FLIR) thermal cameras and there are affordable external thermal cameras that can be connected with smartphones. These cameras provide opportunity to capture thermal transfer and to monitor the speed of the consequent heat dissipation to offer insights of daily interactions with objects and the materials of these objects. %\SystemName{} enhances such possibility, harnessing the residual energy caused by human touch and constructing dissipation fingerprints that characterize how thermal energy dissipates over time.



%We validate \SystemName{} through rigorous benchmark experiments that consider $16$ different objects, that cover most common manufactured materials used in everyday objects and materials.

We validate \SystemName{} through rigorous experiments that consider $14$ different everyday objects that cover the most common materials used in manufactured products. As part of the experiments, we also demonstrate that \SystemName{} generalizes to human temperature variations by considering the robustness of thermal dissipation characteristics of objects with $18$ different individuals. Our results indicate that human-emitted radiation can be used to characterize different materials and that such characterization is robust against variations in individuals and the way they interact with objects themselves. \SystemName{} can determine the correct material with up to $83\%$ accuracy, a $16\%$ improvement on a computer vision baseline that uses deep learning. 
\rev{We also demonstrate that \SystemName{} can characterize materials through other materials and support the simultaneous characterization of multiple objects.}
%for a thickness up to \SI{2}{mm} 
%In this research, We extend \SystemName{} and our previous work~\cite{emenike2021characterizing} to support interactions with multiple objects and analyze the robustness of thermal dissipation fingerprints against covers and other objects that may obscure the camera. Since, off-the-shelf thermal cameras are prone to heating~\cite{flores2019evaluating,malmivirta2019hot}, thus any materials placed in the vicinity to sensor can prevent their capability to capture external interactions. Taken together,
\SystemName{} thus offers an innovative sensing modality that can accurately and robustly characterize everyday objects and enable a broad range of innovative applications.

%, such as waste management and abnormal temperature detection.





\subsubsection*{\textbf{Summary of Contributions}}

\begin{itemize}[noitemsep,leftmargin=*]
\item \textbf{Novel method:} We develop \SystemName{} as a novel sensing approach for characterizing materials using thermal dissipation fingerprints. We demonstrate its usefulness in material classification \rev{and show that \SystemName{} can classify different material types based on the thermal dissipation rate.} %and their characterization, providing a case study for waste material classification. 

\item \textbf{Novel insights:} We demonstrate that current state-of-the-art techniques based on computer vision are limited and only capable of recognizing products that are not mixed with other materials. We also highlight the importance of analyzing objects' material properties to increase robustness of results. 

\item \textbf{Improved performance:} We perform rigorous benchmarks demonstrating that \SystemName{} significantly improves the classification of materials of different sizes and shapes and that is robust across when used among different persons.

% up to \SI{2}{mm} thickness

\item \textbf{\rev{Detection through objects:}} \rev{We demonstrate that \SystemName{} can characterize objects through other materials (up to approximately \SI{2}{\milli\meter} thickness), which increases the practicability and applicability of \SystemName{}. We further highlight this potential by briefly discussing application scenarios that can monitor user interactions through objects or from the internal surfaces of the objects.}

\item \textbf{\rev{Characterization of multiple objects:}} \rev{We extend \SystemName{} to support characterization of multiple objects simultaneously and conduct experiments to analyze the performance of multiple object characterization. The results show that the response time is nearly constant, with increase in the amount of data or the amount of objects having only a marginal impact on response time. In terms of accuracy, the performance depends on how well different objects can be separated, which in turn depends on the constellation of objects and the resolution of the image relative to the objects. }

\end{itemize}



%Besides waste classification, \SystemName{} can also improve other stages in the waste management process.


==> The MIDAS Touch1/sections/MIDASForMultipleObjects.tex <==
%\section{Detecting Multiple Objects} \label{sec:MIDASForMultipleObjects}

\section{Thermal Dissipation Fingerprint for Multiple Objects} \label{sec:MIDASForMultipleObjects}

Our existing prototype and experiments are oriented to the individual characterization of objects using a single thermal dissipation fingerprint. In practice, humans tend to interact with many objects in their vicinity, and thermal dissipation fingerprints of multiple objects need to be analyzed simultaneously. This section describes an extension of the \systemname~pipeline to support the prediction of multiple objects and validates the extended pipeline through benchmark experiments.




\subsection{From Single to Multiple Objects}

When analyzing the thermal fingerprints of multiple different objects, the main challenge is to separate and identify the different objects in the captured image. In thermal imaging, this task is significantly easier than in traditional computer vision. The dissipation of fingerprints is not sensitive to orientation or the shape of an object,  as they are easily distinguishable from the background. However, as shown in Figure~\ref{fig:multipleobjectapproach}a, object arrangement can play an important factor when extracting thermal dissipation vectors. The thermal fingerprint is easily recognizable individually when objects are not touching each other (dispersed), but it can spread over different surfaces if they touch each other (agglomerated).




We extend \systemname~to support multiple objects by including an additional step where the captured image is segmented into regions of interest (ROI)s. The current implementation operates on the normalized grayscale images and detects different ROIs using the~\textit{Counter Approximation Method}\footnote{Available in python CV2 package}; see  Figure~\ref{fig:multipleobjectapproach}b for an illustration. Once the ROIs are detected, each of them is mapped to a dissipation vector that corresponds to one object. As thermal radiation spreads and transfers through the surface of the objects, the identification needs to focus on the centroids of the hottest regions to ensure the ROIs correspond to different objects rather than transfer of dissipating heat along the surface of the object. %the thermal dissipation fingerprints from objects those surfaces are in contact (accumulated) rather than objects that are separated by a distance (disperse).}



\begin{figure}[!t]
	\centering	
	\includegraphics[width=1.0\columnwidth]{graphics/fig12.png}
	\caption{Detection of multiple thermal dissipation fingerprints. a) Object arrangements, b) Extraction of thermal dissipation vectors.}
	\label{fig:multipleobjectapproach}
	   \vspace{-.4cm}
\end{figure}

%\begin{figure}[!t}
%	\centering	\includegraphics[height=10.0cm,width=10.0cm]{graphics/flowchart.png}
%	\caption{Flowchart for Prediction of Material Type.}
%	\label{fig:flowchart}
%	   \vspace{-.4cm}
%\end{figure}

\subsection{Evaluation}

We analyze the performance of our extended approach to recognize multiple objects simultaneously. We measure the degradation in response time when detecting multiple objects in the same images \rev{and we also evaluate the accuracy of the detection}. 

%\textcolor{blue}{We did several experiments regarding the prediction of material type by giving input a videos of equal length and variable length to see the effect response time has when the number of frames are increased.}

\cparagraph{Experimental Setup} The length (time) and frame rate of video footage that captures thermal dissipation are vital factors influencing the accurate identification of multiple objects. \rev{We conduct experiments where we fix the frame rate to $30$fps (i.e., $1800$ frames per minute) and conduct experiments on videos with different length:  (i) four videos of one-minute length; (ii) four videos from $30$ seconds of length to $120$ seconds in $30$ second increments.} In parallel, we also analyze the impact on performance as the number of objects to be identified increases. We analyze the identification from two to four objects simultaneously in different arrangements. Table~\ref{tab:grouping} describes the information on the grouping of object materials. We rely on the household objects used in our previous experiments. Specifically, we used a Coffee Cup (CC), Cigarette Butt (CB), Plastic Bottle (PB), and a Face Mask (mask). 





\begin{table}[h]
\centering
\caption{Table explaining grouping arrangement for prediction of Multiple Objects}
\label{tab:grouping}
\begin{tabular}{@{}|c|l|@{}}
\toprule
\multicolumn{1}{|l|}{\textbf{Arrangement Group}} & \textbf{Description}         \\ \midrule
\textbf{A}                                       & \begin{tabular}[c]{@{}l@{}}One Object at a time. Coffee Cup \includegraphics[height=.5cm ]{graphics/cc.png}, \\ Cigarette Butt \includegraphics[height=.5cm ]{graphics/cigg.png}, \\ Plastic Bottle \includegraphics[height=.5cm ]{graphics/bottle.png}  \end{tabular}                                                 \\ \midrule
\textbf{B}                                       & \begin{tabular}[c]{@{}l@{}}Two Objects at a time. \\ "Coffee Cup + Plastic Bottle" \includegraphics[height=.5cm ]{graphics/cc.png} \includegraphics[height=.5cm ]{graphics/bottle.png}, \\ "Cigarette Butt + Plastic Bottle" \includegraphics[height=.5cm ]{graphics/cigg.png} \includegraphics[height=.5cm ]{graphics/bottle.png}, \\"Coffee Cup + Cigarette Butt" \includegraphics[height=.5cm ]{graphics/cc.png} \includegraphics[height=.5cm ]{graphics/cigg.png} \end{tabular} \\ \midrule
\textbf{C}                                       & \begin{tabular}[c]{@{}l@{}}Three Objects at a time. \\ "Coffee Cup, Plastic Bottle and Cigarette Butt"\\ \includegraphics[height=.5cm ]{graphics/cc.png} \includegraphics[height=.5cm ]{graphics/bottle.png} \includegraphics[height=.5cm ]{graphics/cigg.png}\end{tabular}                        \\ \midrule
\textbf{D}                                       & \begin{tabular}[c]{@{}l@{}}Four Objects at a time. "Coffee Cup, Plastic \\ Bottle, Cigarette Butt and Face Mask \\ \includegraphics[height=.5cm ]{graphics/cc.png} \includegraphics[height=.5cm ]{graphics/bottle.png} \includegraphics[height=.5cm ]{graphics/cigg.png} \includegraphics[height=.5cm ]{graphics/mask.png} 
 \end{tabular}                   \\ \bottomrule
\end{tabular}
\end{table}





\cparagraph{Results - Dispersed case} Figure~\ref{figure:equallengthvideo} shows the results of our first experiment where videos of the same length and frame rate are used. 
\rev{The processing time of the system naturally increases as more dissipation vectors are given as input but the overall increase is negligible. In terms of arrangement of objects, the results similarly are stable, suggesting that the response time of \SystemName{} is not affected by the arrangement of objects -- provided that the dissipation vectors of the materials that form the arrangement can be extracted in a noise-free fashion.}




Figure~\ref{fig:variablelengthvideo} shows the results for the case where different video configurations are considered. \rev{As the length of the video feed increases, the response time of \SystemName{} naturally increases as well. For videos up to $90$ seconds, the length of the video dominates the performance and only once the video length reaches $120$ seconds the impact of segmenting multiple objects becomes visible. In practice the thermal dissipation fingerprints are stable across the video lengths and hence using a short video length of $30$ seconds is sufficient for most situations.} 
%\rev{Figure~\ref{fig:variablelengthvideo}
\rev{The results also show that the response time does not always increase. This is because the response time tends to be dominated by the longest dissipation time and thus cases where one object has significantly longer dissipation time than others tend to have fairly constant response time. Indeed, the response time depends on the calculation of the area reduction in the image. Once the thermal fingerprint has dissipated, the area is effectively zero and the computations return fast. In the experiments, both the plastic bottle and coffee cup have longer dissipation fingerprints than the cigarette butt and thus the response time leans toward the longest vectors.}




\begin{figure}
	\centering
		\includegraphics[width=0.75\columnwidth]{graphics/fig13.png}
	\caption{Response time of multiple object identification when using \systemname. (same video configuration). \rev{The bars within the figure correspond to different individual objects (A) or combination of objects (two objects: B, three objects: C, four objects: D) as given in Table~\ref{tab:grouping}.}}
	\label{figure:equallengthvideo}
\end{figure}




\begin{figure}[!t]
\centering
    \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig14a.png}
   \caption{30 second video (900 frames)}\label{fig:30secsvideo}
  \end{subfigure}   
  \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig14b.png}
    \caption{1 minute video (1800 frames)}\label{fig:1minvideo}
  \end{subfigure} 
  \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig14c.png}
    \caption{1 minute 30 second video (2700 frames)}\label{fig:1min30secsvideo}
  \end{subfigure} 
  \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig14d.png}
    \caption{2 minute video (3600 frames)}\label{fig:2minvideo}
  \end{subfigure} 
  \caption{Impact on response time when using videos of different length and frame rate (Disperse objects case). \rev{The bars within the figure correspond to different individual objects (A) or combination of objects (two objects: B, three objects: C, four objects: D) as given in Table~\ref{tab:grouping}.}} 
  \label{fig:variablelengthvideo}
	   \vspace{-.4cm}
\end{figure}

%\subsection{Multiple Object Detection in Agglomerated Case}

\cparagraph{Results - Agglomerated case} %So far, we have seen \systemname~ can predict and detect multiple objects simultaneously.  our results for multiple object detection are more accurate when the objects are not touching each other \rev{or when they do not overlap each other in such a way such that the thermal dissipation area interfere}. 
\rev{When the objects or the areas of their thermal dissipation area intersect, this can result in dissipation vectors becoming mixed. We next investigate the performance of \systemname{} in such cases.}  %\rev{overlap} each other, their thermal fingerprints 
%also interfere, and our \systemname~model cannot predict the materials with higher accuracy. \rev{In such cases where the objects overlap each other and their thermal dissipation vectors also interfere} the model also fails to predict such materials. 
Figure~\ref{fig:variablelengthvideoagglomerated} shows the processing time of \SystemName{} when materials are in contact. As shown in the figure, we have only considered arrangement groups B,C, and D as we are evaluating multiple objects that are in contact. From the result, we can observe higher computational overhead, which is caused mostly due to the continuous separation of thermal dissipation vectors to characterize individual objects. 

\begin{figure}[!t]
\centering
    \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig15a.png}
   \caption{30 second video (900 frames)}\label{fig:30secsvideoagglomerated}
  \end{subfigure}   
  \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig15b.png}
    \caption{1 minute video (1800 frames)}\label{fig:1minvideoagglomerated}
  \end{subfigure} 
  \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig15c.png}
    \caption{1 minute 30 second video (2700 frames)}\label{fig:1min30secsvideoagglomerated}
  \end{subfigure} 
  \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig15d.png}
    \caption{2 minute video (3600 frames)}\label{fig:2minvideoagglomerated}
  \end{subfigure} 
  \caption{Impact on response time when using videos of different length and frame rate (Agglomerated objects case). \rev{The bars within the figure correspond to different combinations of objects (two objects: B, three objects: C, four objects: D) as given in Table~\ref{tab:grouping}.}} 
  \label{fig:variablelengthvideoagglomerated}
	   \vspace{-.4cm}
\end{figure}

\cparagraph{Effect on Accuracy} \rev{We next assess the effect multiple objects have on the accuracy of \SystemName{}. We only consider the dispersed case as the performance depends on the quality of the segmentation, which is difficult to control systematically. Indeed, in rare cases the segmentation may fail when the thermal fingerprints of two objects appear as a single "blob" in the image, making it impossible to separate them. When the segmentation fails, naturally the following recognition fails.}

\rev{The detection accuracy for multiple object detection is shown in Figure~\ref{fig:accuracy}. For predicting single material objects, the accuracy is $83$\%. For evaluating the effect on accuracy with multiple materials concurrently, we start with combinations based on the arrangement groups from Table~\ref{tab:grouping}. We feed the model with combinations from the different arrangement groups with five different input video footage but involving same combinations to evaluate the average prediction accuracy with multiple materials. We then compare the predictions labels with the true labels and note the average accuracy. For two materials based on arrangement B, the average accuracy achieved was $79.97$\%. For arrangement C with three materials, the average accuracy is $77.75$\% and finally for the arrangement D with four objects, the average accuracy is $61.33$\%. The performance overall depends on the quality of the segmentation, the resolution of the image, and the type of object in the image. As more objects enter the field-of-view, the size of the objects is necessarily smaller than in the case where only a single object is visible. This reduces the quality of the segmentation and the dissipation area, and degrades overall classification performance. Similarly, the four object case is the only configuration that considers the face mask and part of the performance decrease results from difficulty in recognizing the mask. Note that in this type of cases, the objects resulting in poor detection can be separately flagged and they can be analyzed individually to improve the quality of the analysis.}

\begin{figure}
	\centering
		\includegraphics[width=0.75\columnwidth]{graphics/fig16.png}
	\caption{Average prediction accuracy for different number of objects and the corresponding Hamming loss.}
	\label{fig:accuracy}
\end{figure}

%The decrease in the accuracy from evaluating the \SystemName{} on single to multiple material material object detection is obvious as the increase in the number of materials affects the quality of segmentation of region of interests and hence thermal dissipation vectors.}

==> The MIDAS Touch1/sections/MaterialSelection.tex <==
\section{Feasibility Assessment} \label{sec:materialselection}

We first conduct two preliminary studies to demonstrate that heat transfer from humans can be used to characterize different materials and household objects. We capture thermal radiation using COTS smartphone (CAT S60) and validate the measurements using a thermometer scanner that serves as a reference instrument. All statistically significant differences were separately validated using measurements from the reference device. We first describe the testbed setup before detailing the results. 



%by monitoring the resulting thermal radiation and changes in it
\subsection{Testbed}
\label{ssec:testbed}

We capture thermal fingerprints using two devices: a handheld thermal imaging scanner (FLIR TG267) and a Caterpillar smartphone (CAT S60) with an integrated FLIR thermal camera. In all experiments we place the smartphone on a tripod at a distance of \SIrange{30}{35}{cm} % $30-35$ cm 
from the object. We performed manual calibration on the camera after it had attained thermal equilibrium with the environment -- room temperature of \SIrange{22}{23.5}{\degreeCelsius}. %$22-23.5$\textcelsius. 
The video was recorded with the CAT S60, while thermal reference photos were taken with the TG267 scanner. The room's ambient temperature was measured using a Netatmo weather station\footnote{\url{https://www.netatmo.com}}. Dissipation times were estimated automatically from the thermal video and validated by comparing against a ground truth obtained from a manual inspection of the video with a stopwatch. %and manual inspection of the video.

\subsection{Plastic Thermal Fingerprint Dissipation}


\begin{figure*}
	\centering
		\includegraphics[width=1.0\textwidth]{graphics/fig1.jpg}
	\caption{Selected waste materials for preliminary experiments: A (Beer Can), B (Ceramic Cup), C (Takeaway Box), D (Plastic bottle), E (Glass Bottle), F (Coffee Cup), G (Plastic Cup), H(Cigarette Butt), I (Glass Jar), J (Milk pack), K (Aerosol Can), L (Rubber glove), M (Metal spoon) and N (Face mask).}
	\label{fig:EngProto}
\end{figure*}
 

\cparagraph{Experimental Design} We first measure the dissipation time of a thermal fingerprint in different plastic materials and correlate the captured fingerprint with the emissivity coefficient ($\epsilon$) of the material. In this experiment we focus solely on plastics to ensure the emissivity of the materials is known. In subsequent sections, we demonstrate that our solution generalizes to other materials. We consider the most common plastics that can be found in everyday objects: LDPE (Low Density Polyethylene), HDPE (High Density Polyethylene), PP (Polypropylene), PS (Polystyrene), and PVC (Polyvinyl chloride). The material of an object is specified by its Resin Identification Code (RIC), and all materials have well known emissivity coefficients ($\epsilon$=$0.90$ - $0.97$). The tested plastic samples have identical shape and size and have been produced by an identical manufacturing process\footnote{\url{https://www.materialsampleshop.com/products/plastics-sample-set}}. This ensures the samples' differences result from inherent material properties and are not an artifact of any external differences (e.g., shape or stiffness). In the experiments, we first place the plastic sample inside a fridge with a constant temperature of \SI{5}{\degreeCelsius}, to obtain a baseline temperature for comparison. To measure different temperatures, we use a constant heat source (lamp bulb of \SI{60}{\watt}) to heat the plastic samples. The lamp is placed at a fixed distance of \SI{10}{\centi\metre} from the samples to avoid burn damage, ensuring they are exposed to sufficient amounts of thermal radiation. We consider different heating periods ($1$, $2$, $3$ and $4$ minutes) to correspond to differing initial temperatures and measure the dissipation of the thermal fingerprint. \rev{The relative changes in dissipation are highest during the initial minutes and hence periods beyond $4$ minutes were omitted.} During the experiments, ambient temperature oscillated from \SIrange{22}{24}{\degreeCelsius}. %$22-24$\textcelsius. 

% was not necessary for demonstrating a link between dissipation time and the emissivity coefficient.


%We heat the samples during different periods. Once a time period is completed, we remove the heat source and measure the thermal fingerprint dissipation of the plastic sample. Ambient temperature oscillated around $22-24$\textcelsius.

\cparagraph{Results} The results in Figure~\ref{fig:plastics} indicate that the dissipation of thermal fingerprints varies across the materials. The Spearman correlation~\cite{schober2018correlation}  
between dissipation time and emissivity coefficient of the materials was found statistically significant ($\rho=0.66$, p$<.05$), indicating that the dissipation characteristics indeed provide information about the material of the object. 

 


%https://www.ncbi.nlm.nih.gov/pmc/articles/PMC6107969/

\subsection{Other Thermal Fingerprint Dissipations}

%We measure the dissipation of thermal fingerprint via a thermal phone CAT S60, and a certified thermometer CAT TG267. A detailed description of the tested is provided in Section~\ref{sec:experimentalsetup}

%in our experiments that account for a large amount of solid municipal waste~\cite{gundupalli2017multi}. The objects are 

\cparagraph{Testbed} We next demonstrate that the findings of the previous section generalize to other objects and materials by measuring the dissipation time of a thermal fingerprint on different household objects. We consider common household objects, shown in Figure~\ref{fig:EngProto}, including: a beer can (A), ceramic cup (B), takeaway box (C), plastic bottle (D), glass bottle (E), coffee cup (F), plastic cup (G), cigarette butt (H), glass jar (I), milk pack (J), aluminum aerosol can (K), rubber glove (L), steel spoon (M) and a face mask (N). \rev{We measure the dissipation of the thermal fingerprint using a thermal phone CATS60, and a certified thermometer CAT TG267. A detailed description of the apparatus is provided in Section~\ref{sec:experimentalsetup}}.
Similar to our previous experiment, we analyze the thermal dissipation time after the objects are held for $1, 2, 3$, and $4$ minutes. The average body temperature of the human subject holding the object ranged from \SIrange{35}{36}{\degreeCelsius}, and the ambient temperature was from \SIrange{22}{24}{\degreeCelsius}.





\cparagraph{Results} The results in Figure~\ref{fig:allmaterials} are in line with the results for the plastic objects and indicate that the dissipation times differ across the objects and materials. Friedman test using object materials as experimental condition showed the differences of the materials to be statistically significant ($\chi^2(2)=48.83$, $p<.05$, $W=0.93$), demonstrating that thermal radiation can indeed characterize different object materials. 





\begin{figure*}[!t]
\centering
    \begin{subfigure}[b]{0.32\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig2a.png}
    \caption{}\label{fig:plastics}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig2b.png}
  \caption{}\label{fig:allmaterials-thermometer}
 \end{subfigure}  
 \begin{subfigure}[b]{0.32\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig2c.png}
    \caption{}\label{fig:allmaterials-cat60}
 \end{subfigure} 
 \caption{Dissipation time of thermal fingerprints in different plastic materials and waste material using two different devices: (a) Grouped by RIC code, (b) Thermometer scanner FLIR TG267 (baseline), and (c) Smartphone CAT s60.}
 \label{fig:allmaterials}
 \vspace{-.4cm}
\end{figure*}









==> The MIDAS Touch1/sections/Model.tex <==
\section{\SystemName{} Pipeline}
\label{sec:methodology}

Aforementioned results demonstrated that dissipation of thermal fingerprints provides information that can be used to characterize different objects and identify their materials. We next briefly describe the sensing pipeline used as a solution to characterize everyday objects. \SystemName{} takes a sequence of thermal images taken from the object's surface as input and returns an estimate of the most likely material of that object. Next we describe the thermal image model which is used to classify object materials based on the dissipation time of thermal fingerprints.

\begin{figure}
	\centering
		\includegraphics[width=\columnwidth]{graphics/fig3.png}
	\caption{Dissipation time of thermal fingerprint for two different objects: (a) Cardboard cup and (b) Cigarette butt.}
	\label{fig:fading}
\end{figure}

\cparagraph{Preprocessing and Normalization} Since COTS thermal cameras are without cooling, they suffer from inaccuracies resulting from the camera overheating~\cite{malmivirta2019hot}. Other factors that influence measurement quality include misalignment between thermal and RGB pictures, internal recalibration of the camera, and low resolution. To mitigate these effects, we preprocess the thermal camera data by examining the background of consecutive images and removing images with significant dissimilarities. We also apply denoising on the images, normalizing the thermal values to a consistent scale (between $0$ and $255$). Such allows us to manipulate the images in gray scale. Figure~\ref{fig:fading} depicts the result of normalization procedure. The figures shows the sequence of thermal pictures over time (upper) and the corresponding image on the normalized scale (below) for two objects: (a) a cardboard cup and (b) a cigarette butt. This allows to isolate the thermal fingerprints from each object. 



\cparagraph{Dissipation Rate} We estimate the dissipation rate of the thermal fingerprint from the normalized sequence of pictures as the function of area reduction of the thermal fingerprint given by the equation: 
\begin{equation}
RA = (A_{i} - A_{t})/A_{i},
\label{eq:reduction-area}
\end{equation}
\noindent where $RA$ is the reduction area percentage, $A_{i}$ is the initial area, and $A_{t}$ is the reduced target area~\cite{national2003fundamentals} (see Figure~\ref{fig:fading}). The reduction area between consecutive images is used to create vectors that model the dissipation time of thermal fingerprints for each object. \rev{To facilitate the training of machine learning classifiers, we consider fixed sized vectors. Note that once the fingerprint has dissipated, the target area is zero and thus this effectively corresponds to padding the vector with zeroes.} 





\cparagraph{Implementation} Vectors with dissipation time are used as feature vectors and the type of object as label class. We then construct classification models using common machine learning techniques: Random Forests (RF), Support Vector Machines (SVM), and Multi-Layer Perceptron Classifier (MLPC).









==> The MIDAS Touch1/sections/Motivation.tex <==
\section{Motivation}
\label{sec:motivation}

\begin{figure}[!t]
\centering
    \begin{subfigure}[b]{.34\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/waste3.png}
   \caption{}\label{fig:waste1}
  \end{subfigure}   
  \begin{subfigure}[b]{.42\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/waste4}
    \caption{}\label{fig:waste2}
  \end{subfigure} 
  %\vspace{-15pt}
  \caption{Trained model PlasticNet, discriminating plastics against other object materials~\cite{prata2020covid}} 
  \label{fig:computer-vision}
\end{figure}



We begin by demonstrating how existing sensing techniques based on automated computer vision~\cite{white2020wastenet,ruiz2019automatic} and light sensing~\cite{singh2016iot} fail in identifying material properties and objects in general. \SystemName{} has been designed to overcome the limitations of these techniques by using material properties as the means for characterizing objects. 


\subsection{Computer vision analysis}

\cparagraph{Experiment} We first attempt to classify household objects using computer vision and train a state-of-the-art Convolutional Neural Networks (CNNs) model using the publicly available TrashNet dataset~\cite{aral2018classification}. We focus exclusively on the plastic materials category which contains $626$ images of plastic objects for training the deep learning model. Plastics are malleavable, so their accurate recognition is very sensitive to changes. The dataset has images where the individual pieces are shown against a white background. As such images do not match realistic recognition settings, we supplement the dataset with an additional $767$ images from the Japan Agency for Marine Earth Science and Technology (JAMSTEC) Deep-sea Debris Database dataset. %(additional 767 images).
%it was expected that such imagery would not match the real case of tossed and squashed waste against the background (e.g., pavement). For those reasons, we added 

Collected images were annotated manually by drawing a rectangle box around the object material in images. We labeled the TrashNet plastic items as "trash" and the JAMSTEC plastic items as "plastic". Both datasets were augmented by adding noise, hue, blue, horizontal flip, and vertical flip modifications to each original image, resulting in a total of 6985 for model training input. We created and trained the PlasticNet model using Google Collab server GPU, with 100k iterations and a batch size of 12, running TensorFlow Lite 1.15. For the base training model, ssd\_mobilenetv2\_oidv4 was used.

\cparagraph{Results} For validation, we used 31 images depicting real tossed plastic objects~\cite{prata2020covid}. In total, 33 separate plastic items were present in the 31 images. The deep learning model managed to identify 23 of the 33 items, obtaining 69.7\% in accuracy. Figure~ \ref{fig:computer-vision} highlights the main limitation of the model, being unable to identify multiple objects simultaneously and objects whose shape changes drastically. Although the trained model was primarily focused on plastics, such findings suggest that the application of using deep learning models and image vision for real life tossed object materials remains limited. 




\subsection{Light reflectivity analysis}
\cparagraph{Experiment} Reflectivity analysis of materials is a highly adopted technique to classify different material types~\cite{singh2016iot}. We next classify materials using light reflectivity measured through a photoresistor connected to the analog input pin of an Arduino MEGA ADK. The photoresistor captures light changes based on its resistance exposure to the light intensity of the reflected material. As a light source, we rely on a red laser diode (wavelength $650$ nm). The object was located $2$ cm away from the light source, depicting a practical usage of the sensor in transport belts and smart bins~\cite{white2020wastenet}. We took measurements with the sensor for different materials (selection described in Section~\ref{sec:materialselection}) during $1$ min from two different places of the object selected randomly. 

\cparagraph{Results} Figure~\ref{fig:Light-reflectivity} depicts the results and compares them to two baseline backgrounds (white and black). We can observe that light can characterize different materials with low variations, but that different parts of the same material can be characterized very differently, e.g., Cardboard Cup-1 and Cardboard Cup-2. This is because objects (end-products) consist of different materials and colors, both affecting its properties. A key limitation is that this approach requires a very short distance between the material and the sensor to classify the material accurately. Another limitation is that the light beam can cover a limited area, leaving most of the object untreated. 
 
\begin{figure}
	\centering
		\includegraphics[width=0.7\columnwidth]{graphics/Material-reflection-laser.eps}
	\vspace{-15pt}	
	\caption{Light reflectivity values of different materials measured with a photo-resistor.}
	\label{fig:Light-reflectivity}
\end{figure}

==> The MIDAS Touch1/sections/RelatedWork.tex <==
\section{Related Work}




\cparagraph{Thermal imaging}
% Objects with a temperature above absolute zero (-273$^{\circ}$C) emit infrared radiation, for which Infrared Thermal Imaging (ITI, or thermography) is used to detect it~\cite{vollmer2017infrared}. ITI occurs beyond the red end of the visible light spectrum (infrared wavelength range $0.78-1000\mu m$~\cite{mehta2011introduction,kruse2001uncooled}), where thermal cameras are used to detect it in $2 - 14\mu m$~\cite{abdelrahman2017cognitive} bands, monitoring temperatures from -50 to 2000$^{\circ}$C.
The usage of thermal imaging has been studied in different domains and applications with examples ranging from monitoring the manufacturing process of smartphone hardware components~\cite{xie2014therminator} to medical analysis~\cite{sun2011portable,harangi2011detecting}. Other examples include facial recognition for bio-metric authentication~\cite{bhowmik2008classification}, cognitive analysis~\cite{abdelrahman17cognitive}, gestures~\cite{larson2011heatwave, abdelrahman2015investigation}, and energy modeling of IoT devices~\cite{flores2019evaluating}. Our work extends thermal imaging to material classification. 

%use it to discriminate waste materials, exploring Thermal Dissipation Fingerprint, a human-emitted thermal radiation transferred from persons to objects. 

 %Other applications of thermal imaging include agriculture~\cite{vadivambal2011applications}, and human-assisted intelligent systems, e.g., fire detection~\cite{hwang2010novel, arrue2000intelligent}.

\cparagraph{Material sensing} Materials have different characteristics different properties that can be exploited to categorize them. The most common material sensing approach is to rely on different parts of the light spectrum and measure either reflection or absorption at different frequencies. Examples range from the use of green light sensing to detect plastic waste~\cite{flores2020penguin} to the use of near-infrared sensing to facilitate medicine adherence~\cite{klakegg2018assisted} and the use of hyperspectral imaging for estimating sugar content in drinks~\cite{jiang2019probing}. Also, deep learning approaches for detecting different material types from reflection patterns at different wavelengths have been proposed~\cite{cho2018deep}. %A key limitation of existing imaging techniques is that they focuses on external characteristics of reflection or absorption which are dependent on the shape, color and other properties of the items rather than capturing only intrinsic characteristics of the materials themselves. 
%Our work extends these works by using infrared spectrum to estimate internal characteristics of materials related to heat dissipation.
Our work extends these by using thermal radiation in the infrared spectrum to estimate internal characteristics of materials through heat dissipation.



%\cparagraph{Batteryless sensing}
\cparagraph{Sensorless sensing} %Besides using wireless signals to infer the surroundings in an environment~\cite{zhou2015sensorless} and users' activities~\cite{wu2017device}, 
Wireless signals can also be used to identify properties in materials. Examples include the use of variations in WiFi signal propagation characteristics to identify liquids~\cite{dhekne2018liquid}, and the use of surface tension to characterize liquids~\cite{yue2019liquid,wei2015study}. These methods generally require either close contact with the material or a transmitter - receiver pair to be placed on opposite sides of the material. Our work offers a non-contact technique for material characterisation that piggybacks thermal radiation generated from humans. %to enable a sensing modality that characterizes material based on dissipation patterns captured in the infrared spectrum solely. 




==> The MIDAS Touch1/sections/Results.tex <==
\section{Results} \label{sec:results}

%http://www.easysurf.cc/scintd.htm

%In forthcoming, 
We next demonstrate that \SystemName{} can characterize different object materials accurately using the measurements from the controlled user evaluation described in the previous section. We consider robustness against variations in the way humans interact with objects and variations in individuals, the overall classification performance for different materials, \rev{and the robustness of the detection to operate through other objects.}

%
%and (iii) practicability of our approach with a use case of recognizing abnormal human temperature.

%different object materials. We conduct a controlled study with multiple participants in a lifespan of two weeks. The objective is to determine whether it is possible to use human-emitted thermal radiation to characterize different objects. By relying on different human subjects, we expect to learn whether our approach can be generalized across different objects and users.






%We found statistically significant differences between forehead/hand-palm ($p=0.0002$) and forehead/finger-tips ($p=0.0002$), but no differences between hand-palm/finger-tips ($p=0.052$). From the results, we can observe a difference of $4-6$\textcelsius~between forehead and hand-palm/finger-tips, and higher variance for hand-palm/finger-tips measurements. This can indicate that hand-palm/finger-tips are more susceptible to ambient temperature changes and can also capture more indirect insights about activities that users are performing. For instance, the battery temperature from a  smartphone can induce a higher temperature in an individual, indicating the level of smartphone usage \cite{}. Induced temperature can help situations where the environment inhibits human-emitted radiation transferred to object materials, e.g., cold temperatures below $0$\textcelsius. 


%While results indicate a difference of $4-6$\textcelsius~between forehead and hand-palm/finger-tips, we can observe that temperatures of each body part in general are constant and do not  


%\begin{figure}
	%\centering
%		\includegraphics[width=0.7\columnwidth]{graphics/Participants-temperature.eps}
%	\caption{Body temperature of the  participants.}% in different body parts.}
%	\label{fig:body-parts-temperature}
%	   \vspace{-.4cm}
%\end{figure}



%\subsection{Human-emitted thermal radiation to objects}
\subsection{Differences in Thermal Fingerprints}

We first examine differences in thermal transfer from humans and the ensuing dissipation in the different objects. We separately consider the impact of the object and the hold type on thermal transfer. 

%\cparagraph{Hold type differences}
The dissipation times of the three objects under the different hold type conditions are shown in Figure~\ref{fig:dissipation}. From the figure, we can observe the differences in objects to be consistently different regardless of the hold type. Friedman Test using dissipation time and objects as experimental conditions shows the differences in objects to be significant for all of the three hold-type conditions: Fixed-hold ($\chi^2(2)=20.33$, p~$<.05$, $W=0.56$), Natural-hold ($\chi^2(2)=30.33$, p~$<.05$, $W=0.84$) and Quick-hold ($\chi^2(2)=25.04$, p~$<.05$, $W=0.64$). Pairwise post-hoc comparisons using Wilcoxon test (with Bonferroni correction for multiple comparisons) confirmed that the differences in dissipation times are statistically significant for all object pairs across the three hold types.

%\cparagraph{Hold type and materials}
We next assess how the hold type affects the thermal fingerprints. % the differences in the characterization of the same object between different conditions to determine the factors that influence the characterization process. 
Friedman test using dissipation time of each object and the three experimental conditions shows hold type to result in significant differences %for a small difference between conditions for cigarette-butt ($\chi^2(2)=1$, p-value $=0.6$, W=$0.027$), a moderate difference 
for the plastic bottle ($\chi^2(2)=12.44$, p $<.05$, W=$0.34$) and the cardboard cup ($\chi^2(2)=16.48$, p $<.05$, W=$0.45$), but not for the cigarette butt. Post-hoc comparisons indicate the thermal fingerprints for the Quick-hold pattern to significantly differ from those in the Fixed- and Natural- hold conditions. Results imply that \textit{differences} in thermal fingerprints contain significant variation across objects regardless of how users touch or interact with them. Still, the dissipation times are impacted by the time the user holds the item. This is expected, as the time the user touches the object affects the extent of heat that can transfer and thus controls dissipation speed.

We also separately analyzed whether differences in body temperature across different body parts can affect the thermal fingerprint by comparing the thermometer results across the three measurement locations (forehead, hand palm, finger tips). Friedman test using part of body as experimental conditions showed significant differences for temperature ($\chi^2(2)=29.66$, $p<.05$, $W=0.82$). Post-hoc comparisons (Dunn-Bonferroni) verified that the differences were statistically significant ($p<.01$) between forehead and hand-palm and between forehead and finger-tips. The average temperature for the different parts of body were: forehead \SI{36.33}{\degreeCelsius}, hand-palm \SI{30.16}{\degreeCelsius}~and finger-tips \SI{30.87}{\degreeCelsius}. % To quantify the effect of these differences, we calculate Kendall's W coefficient. The result ($W=0.82$) indicates the presence of a large effect in concordance with Cohen's interpretation guidelines ($W=0.82$). We also calculate a pairwise Wilcoxon test\footnote{p-values are adjusted using the Bonferroni multiple testing correction method, significance p-value $<.01$} to identify which body parts depict different temperatures. We found statistically significant differences between forehead/hand-palm (p-value $<.01$) and forehead/finger-tips (p-value $<.01$), but no differences between hand-palm/finger-tips ($p=0.052$).
These results show that fingers and hand palm generally induce similar heat transfer, further validating the robustness of the thermal fingerprints against the way people interact with the objects. The difference to forehead temperature, in turn, suggests that the hand palm and fingertips react to ambient temperature instead of correlating with the internal body temperature -- as is the case for the forehead measurements. We note that the higher sensitivity of finger tips and hand palm also means that it can be potentially used to extract insights about human activity. For example, interactions with a smartphone can result in heat caused by battery temperature to transfer into the hand, and the contents of a hot drink can similarly affect the temperature.  %Induced temperature can also help in situations where the environment inhibits human-emitted radiation transferred to object materials, e.g., temperatures below \SI{0}{\degreeCelsius}. 

%Forehead temperature typically correlates strongly with actual body temperature, and hence the results show that the thermal fingerprints do not necessarily provide sensitive information about body temperatureas these locations are more sensitive to variations in ambient temperature. 

%These results show that hand palm and finger tips generally have similar temperature, further suggesting that the way people grasp the objects does not affect the performance of \SystemName{}. The forehead temperature is significantly different from the  

%From the results, we can observe a difference ranging from \SIrange{4}{6}{\degreeCelsius} between forehead and hand-palm/finger-tips, and higher variance for hand-palm/finger-tips measurements. This can indicate that hand-palm/finger-tips are more sensitive to ambient temperature changes and can also capture more indirect insights about the users' activities. For instance, the battery temperature from a smartphone can induce a higher temperature in an individual, indicating the level of smartphone usage~\cite{sarsenbayeva2017sensing}. 

Overall, the results indicate that human touch transfers a sufficient amount of heat, making it possible to characterize objects based on touch without resorting to specialized technology. However, the results show that the dissipation times are affected by the time the user interacts with the objects -- and other factors as will be shown in the next subsection -- implying that relative differences in dissipation characteristics should be used instead of the exact dissipation times for characterizing materials. 



%\subsection{Validity: Body Temperature and Thermal fingerprint}

%Figure~\ref{fig:body-parts-temperature} shows the body temperatures from all the participants for different body parts.
%In the experiments we consider thermal fingerprints resulting from human touch. Before analyzing the dissipation characteristics in detail, we demonstrate that the variations between hand palm and finger tips are sufficiently small to 

%In the experiments we have relied on objects that people touch with their hand palms and finger tips. To validate this choice, we analyzed variations in human body temperature by comparing 


%These results imply that thermal radiation fingerprints resulting from natural interactions with everyday objects can be further exploited to characterize different materials.



%Our results thus indicate that the hand palm and finger tips can transfer sufficient amounts of heat to characterize different materials regardless of the way people touch and interact with the objects. This implies that we can fingerprint different materials simply using human touch without resorting to specialized technology.


%We first investigate the differences in thermal dissipation across objects and how the hold-type affects it. We accomplish this by analyzing thermal radiation transferred from hand palm and finger tips to the object, and measuring the dissipation time of the thermal fingerprint under in three different experimental conditions. The dissipation times are shown in Figure~\ref{fig:dissipation}.
%To determine whether the dissipation time of thermal radiation is different for different object materials, we calculate their statistical differences using the Friedman test. When objects were exposed to a fixed-hold condition, our results indicate that the dissipation time for different objects is statistically different ($\chi^2(2)=20.33$, p-value $<.05$, $W=0.56$).  %between bottle/cigar (p-value $<.01$), bottle/cup (p-value $<.01$) and cigar/cup (p-value $<.01$) are significant. 
%Similarly, when thermal radiation was transferred to an object using a Natural-hold, our results also indicate that the dissipation time for different objects is statistically different ($\chi^2(2)=30.33$, p-value $<.05$, $W=0.84$). %In addition, pairwise Wilcoxon test also confirms that dissipation time between bottle/cigar (p-value $<.01$), bottle/cup (p-value $<.01$) and cigar/cup (p-value $<.01$) are significant. 
%By relying on a Quick-hold condition, we also estimate the dissipation time when thermal radiation was transferred in a short period. Our results indicate that the dissipation time for different objects is statistically different ($\chi^2(2)=25.04$, p-value $<.05$, $W=0.64$). 
 %, but instead, just by relying on a simple human touch with much anticipation. This has potential because the fingerprinted objects do not need to pass through complex waste management routines to obtain their material characteristics. 



%Next, we analyze the thermal radiation transferred from hand-palm/finger-tips to object materials as thermal fingerprints. To do this, We analyze the dissipation time of the thermal fingerprint from the three object materials under our three experiment conditions (Fixed-Hold, Natural-Hold, and Quick-hold). Figure~\ref{fig:dissipation} shows the dissipation time for all the conditions. To determine whether the dissipation time of thermal radiation is different for different object materials, we calculate their statistical differences using Friedman test. When objects were exposed to a fixed-hold condition, our results indicate that the dissipation time for different objects is statistically different ($\chi^2(2)=20.33$, $p=3.84e-05$) with a large quantifiable effect ($W=0.56$). In addition, pairwise Wilcoxon test also confirms that dissipation time between bottle/cigar ($p=0.0002$), bottle/cup $p=0.0002$ and cigar/cup $p=0.0008$ are significant. Similarly, when thermal radiation was transferred to an object using a Natural-hold, our results also indicate that the dissipation time for different objects is statistically different ($\chi^2(2)=30.33$, $p=2.58e-07$) with a large quantifiable effect ($W=0.84$). In addition, pairwise Wilcoxon test also confirms that dissipation time between bottle/cigar ($p=7.63e-06$), bottle/cup $p=4.93e-04$ and cigar/cup $p=3.00e-04$ are significant. By relying on a Quick-hold condition, we also estimate the dissipation time when thermal radiation was transferred in a short period. Our results indicate that the dissipation time for different objects is statistically different ($\chi^2(2)=25.04$, $p=3.64e-06$) with a large quantifiable effect ($W=0.64$). In addition, pairwise Wilcoxon test also confirms that dissipation time between bottle/cigar ($p=0.0002$), bottle/cup $p=0.001$ and cigar/cup $p=0.01$ are significant. Our results indicate that enough thermal radiation can be found in hand-palm/finger-tips to characterize different materials for all conditions. These results also suggest that object materials can be fingerprinted without relying on any specialized technology, but instead, just by relying on a simple human touch with much anticipation. 


%This results indicates that in any condition, there is dissipation time can be used to characterize different objects.




%\subsection{Differences between thermal transferred conditions}

%Previously, we demonstrated the possibility to characterize objects with thermal human-emitted radiation for each of our experimental conditions. In this section,  we analyze the differences in the characterization of the same object between different conditions. We aim to determine the factors that influence the characterization process. To do this, we compare the dissipation time of each object. For the cigarette butt, the Friedman test indicates a small difference between conditions ($\chi^2(2)=1$, $p=0.6$, Kendall´s W=$0.027$). Moreover, pairwise Wilcoxon test indicates no significant differences between the three thermal transferred conditions, fixed/natural ($p=0.79$), fixed/quick ($p=0.14$) and natural/quick ($p=0.07$). This suggests that the characterization of the object with thermal radiation does not depend on the transferred time nor the transfer location. Naturally, since the cigarette-butt's overall size is small, the thermal radiation is concentrated and retained in a specific area. Likewise, for the plastic bottle, Friedman test indicates a moderate difference between the three conditions ($\chi^2(2)=12.44$, $p=0.001$, Kendall´s W=$0.34$). Moreover, the pairwise Wilcoxon test indicates no significant differences between fixed and natural conditions ($p=0.38$). However, significant differences were found between fixed/quick ($p=0.0004$) and natural/quick ($p=0.005$). This result indicates that the absorption of thermal radiation for the object is slow and depends on the exposure time. Conversely, this result also indicate that the location is not a relevant factor (as long as the material is the same) to quantify the dissipation time. Thus, thermal radiation can be used to characterize objects that are held in a natural way by people. Lastly, for the cupboard cup, the Friedman test indicates a moderate difference between the three conditions ($\chi^2(2)=16.48$, $p=0.0002$, Kendall´s W=$0.45$). Moreover, the pairwise Wilcoxon test indicates no significant differences between fixed and natural conditions ($p=0.36$). However, significant differences were found between fixed/quick ($p=0.0003$) and natural/quick ($p=0.005$). This result confirms that the characterization of objects with thermal radiation depends on the exposure time and does not depend on the location or area that the thermal radiation can cover. 

%conditions for the plastic bottle (fixed cf. quick and natural cf. quick) and the cardboard cup (fixed cf. quick and natural cf. quick). The results suggest that the characterization of the object with thermal radiation neither tied to an unnatural manner of interacting with objects nor to a specific area location on the object (e.g., since the cigarette-butt's overall size is small, the thermal radiation is concentrated and retained in a specific area). The absorption of thermal radiation for some objects (e.g., plastic bottles) is slow and depends on the exposure time. Conversely, this result also indicates that the location is not a relevant factor (as long as the material is the same) to quantify the dissipation time. Thus, thermal radiation can be used to characterize objects that are held naturally by people. In general, our results indicate that the characterization of objects with thermal radiation depends on the exposure time and does not depend on the location or area that the thermal radiation can cover. Therefore, the natural interactions with objects can be exploited to identify materials with thermal radiation. 

%To do this, we compare the dissipation time of each object. For the cigarette butt, the Friedman test indicates a small difference between conditions ($\chi^2(2)=1$, p-value $=0.6$, Kendall´s W=$0.027$). Moreover, pairwise Wilcoxon test indicates no significant differences between the three thermal transferred conditions, fixed/natural (p-value $>.01$), fixed/quick (p-value $>.01$) and natural/quick (p-value $>.01$). This suggests that the characterization of the object with thermal radiation is not tied to an unnatural manner of interacting with objects nor an specific area location in the object. Naturally, since the cigarette-butt's overall size is small, the thermal radiation is concentrated and retained in a specific area.
%Likewise, for the plastic bottle, the Friedman test indicates a moderate difference between the three conditions ($\chi^2(2)=12.44$, p-value $<.05$, Kendall´s W=$0.34$). Moreover, the pairwise Wilcoxon test indicates no significant differences between fixed and natural conditions (p-value $>.01$). However, significant differences were found between fixed/quick (p-value $<.01$) and natural/quick (p-value $<.01$). This result indicates that the absorption of thermal radiation for the object is slow and depends on the exposure time. Conversely, this result also indicates that the location is not a relevant factor (as long as the material is the same) to quantify the dissipation time. Thus, thermal radiation can be used to characterize objects that are held naturally by people.
%Lastly, for the cupboard cup, the Friedman test indicates a moderate difference between the three conditions ($\chi^2(2)=16.48$, p-value $<.05$, Kendall´s W=$0.45$). Moreover, the pairwise Wilcoxon test indicates no significant differences between fixed and natural conditions (p-value $>.01$). However, significant differences were found between fixed/quick (p-value $<.01$) and natural/quick (p-value $<.01$). This result confirms that the characterization of objects with thermal radiation depends on the exposure time and does not depend on the location or area that the thermal radiation can cover. Taken together, our results indicate that natural interactions with objects can be exploited to fingerprint materials through thermal radiation dissipation. 


%This suggests that the characterization of the object with thermal radiation does not depend on the transferred time nor the transfer location.



\begin{figure*}[htb]
\centering
    \begin{subfigure}[b]{.3\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig7a.png}
   \caption{Fixed-hold}\label{fig:fixedhold}
  \end{subfigure}   
  \begin{subfigure}[b]{.3\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig7b.png}
   \caption{Natural-hold}\label{fig:naturalhold}
  \end{subfigure}   
  \begin{subfigure}[b]{.3\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig7c.png}
    \caption{Quick-hold}\label{fig:quickhold}
  \end{subfigure} 
  \caption{Thermal transferred conditions applied over three different objects (plastic bottle, cardboard cup and cigarette butt).} 
  \label{fig:dissipation}
\end{figure*}




\subsection{Other Factors Influencing Thermal Dissipation}

%As temperature directly impacts the thermal radiation of objects, we analyze further differences in temperature between participants to identify other factors that influence the thermal radiation transferred. 

Thus far we have shown that the characterization of object materials with thermal radiation depends on exposure time, but not on the location where the object is being touched at. In this section, we investigate other factors that influence the transfer of thermal radiation from the human body to objects.

%\cparagraph{Female vs male temperature} As body temperature directly influences the thermal radiation transferred to objects, we analyze whether temperature differences between female and male participants were significant for thermal transfer. Figure~\ref{fig:gender} shows the results for each body part, forehead, hand-palm, and finger-tips. To determine differences between the two groups, we ran Kruskal-Wallis test\footnote{significance $p<0.05$}. The result shown that there are significant differences for finger-tips ($\chi^2(2)=5.08$, $p=0.02$), but no differences in hand-palm ($\chi^2(2)=1.87$, $p=0.17$) and forehead temperatures ($\chi^2(2)=0.097$, $p=0.75$). When analyzing the cigarette-butt, Kruskal-Wallis test indicates significant differences in the dissipation time ($\chi^2(2)=3.94$, $p=0.04$). The Kruskal-Wallis test also indicated significant differences in the dissipation time for plastic bottles ($\chi^2(2)=12.17$, $p=0.0004$) and cardboard cup ($\chi^2(2)=7.75$, $p=0.005$). These results indicate that the dissipation time of the thermal fingerprint depends on temperature and that it is possible to identify whether a female or male individual touched the object.  

 %Figure~\ref{fig:gender} shows the results for each body part, forehead, hand-palm, and finger-tips. 
 
 



\cparagraph{Gender and Temperature} Body temperature generally influences thermal radiation transferred to objects. We next analyze whether the gender of the participants affects thermal transfer, i.e., whether there are significant differences in thermal transfer between female and male participants. We separately assessed effects for the hand palm and finger tips. Kruskal-Wallis tests, using gender and part of the body as experimental conditions, show that there are significant differences in thermal transfer only for finger tips ($\chi^2(2)=5.08$, p $<.05$). This is most likely the result of differences in the size of the contact area with males typically having larger fingertip size~\cite{acree1999there}.

%, but no differences in hand-palm ($\chi^2(2)=1.87$, p-value $>.05$) and forehead temperatures ($\chi^2(2)=0.097$, p-value $>.05$).
%To determine differences between the two groups, we ran the Kruskal-Wallis test\footnote{Kruskal-Wallis significance p-value $<.05$}. The result has shown that there are significant differences for finger-tips ($\chi^2(2)=5.08$, p-value $<.05$), but no differences in hand-palm ($\chi^2(2)=1.87$, p-value $>.05$) and forehead temperatures ($\chi^2(2)=0.097$, p-value $>.05$).

When using gender and objects as experimental conditions, Kruskal-Wallis tests show there to be significant differences in the dissipation time for all three objects: cigarette butt ($\chi^2(2)=3.94$, p $<.05$), plastic bottle ($\chi^2(2)=12.17$, p $<.05$) and cardboard cup ($\chi^2(2)=7.75$, p $<.05$).
%When analyzing the cigarette-butt, Kruskal-Wallis test indicates significant differences in the dissipation time ($\chi^2(2)=3.94$, p-value $<.05$). The test also indicated significant differences in the dissipation time for plastic bottles ($\chi^2(2)=12.17$, p-value $<.05$) and cardboard cup ($\chi^2(2)=7.75$, p-value $<.05$). 
These results indicate that the thermal fingerprint's dissipation time depends on temperature and that it is possible to identify whether a female or male individual has touched the object. While this result does not change the fact that objects can be characterized with thermal radiation, \rev{it is also important to highlight the potential privacy implications. Indeed, the results show that thermal radiation can disclose additional information about the humans interacting with the objects.} For example, it could be possible to use thermal fingerprints to compare household waste sorting practices between genders.  

%persuasive stimuli that make females or males more prone to dispose of waste in the right recycling trash bin. 

%\begin{figure}[!t]
%\centering
    %\begin{subfigure}[b]{.45\linewidth}
    %\centering
    %\includegraphics[width=1.0\textwidth]{graphics/Participants-female-temperature.eps}
   %\caption{Female participants}\label{fig:female}
  %\end{subfigure}   
  %\begin{subfigure}[b]{.45\linewidth}
    %\centering
    %\includegraphics[width=1.0\textwidth]{graphics/Participants-male-temperature.eps}
    %\caption{Male participants}\label{fig:male}
  %\end{subfigure} 
  %\caption{Differences in body temperature parts for female and male participants.} 
  %\label{fig:gender}
%\end{figure}
% of \SI{5}{\degreeCelsius}, to

\cparagraph{External Temperature of Ambient Environment} Surrounding temperature of the object directly influences the dissipation time of the thermal fingerprint. We quantity the influence of this factor through additional small scale experiments. First, the BOTTLE was held by a human hand for different periods at an ambient temperature of \SIrange{22}{23.5}{\degreeCelsius}. Next, the BOTTLE was placed inside a colder environment (fridge with a temperature of \SI{5}{\degreeCelsius}). We then measured the dissipation time of the thermal fingerprint when changing from ambient to colder environment using both the CAT S60 and the thermometer scanner. Figure~\ref{fig:factors} shows the results. We also include the thermal fingerprint's dissipation time in the ambient environment for comparison purposes (baseline). We notice the total dissipation time of the thermal fingerprint is halved when changing to a colder environment. Still, overall the differences in change patterns remain consistent for the different objects. This suggests that the environment affects the fingerprints. Note that the magnitude of this change is proportional to heat difference and impacts all objects equally. Hence, incorporating the ambient temperature in the thermal dissipation fingerprints is sufficient to overcome potential issues from differing temperatures.  %This suggests that environment is a key factor to monitor when relying on thermal fingerprints to fingerprint materials.


\cparagraph{Internal Temperature absorbed from Contents} Besides the ambient temperature of the surrounding environment, objects can also be influenced by the thermal radiation resulting from the contents of the object. For example, a cardboard cup can be filled with a hot or a cold drink. To investigate this further, we fill the BOTTLE with water with a temperature of \SIrange{21.2}{21.5}{\degreeCelsius}. Before the experiment, we place the BOTTLE inside a fridge (\SI{5}{\degreeCelsius}) to eliminate thermal radiation carryover effects between experiments. We then compare the dissipation times of an empty and filled bottle in ambient temperature (\SIrange{22}{23.5}{\degreeCelsius}). Figure~\ref{fig:factors} depicts the results. We observe that the internal radiation impacts the thermal fingerprint of the BOTTLE. This is relevant to identify end-products that have not been fully consumed. In practice, such cases should be modeled as a separate (mixed) object to ensure the model can distinguish the pure material from those cases where there are no contents inside the object. Compared with the thermal fingerprint of the empty BOTTLE, we can observe that the thermal fingerprint of the filled water BOTTLE dissipates faster as a result of the larger difference with the environment. 

%This is because the water became colder with time from the acquisition of the baseline temperature, and colder water accelerated the BOTTLE's dissipation time. 



\begin{figure}[!t]
\centering
    \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig8a.png}
   \caption{CAT s60}\label{fig:bottle-cats60}
  \end{subfigure}   
  \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig8b.png}
    \caption{Thermometer Scanner}\label{fig:bottle-thermometer}
  \end{subfigure} 
  \caption{Influence of internal and external temperatures.} 
  \label{fig:factors}
	   \vspace{-.4cm}
\end{figure}


\cparagraph{Distance between Object and Thermal Camera} In the experiments thus far, the distance between the thermal camera and the objects has been fixed at \SIrange{30}{35}{\centi\metre} (baseline). We next analyze the effect of longer distances by considering three additional distances: \SI{70}{\centi\metre} (distance-1), \SI{105}{\centi\metre} (distance-2) and \SI{210}{\centi\metre} (distance-3). %We chose these distances as they enable us to measure thermal fingerprints from both the CAT S60 and the thermometer scanner. 
We focus exclusively on the BOTTLE with a Fixed-hold setup of one minute. At \SI{70}{\centi\metre} distance, the dissipation time does not change significantly (average time = $1.13$ min) for the CAT S60. At longer distances, we observed higher variations in the dissipation time with the CAT S60. At \SI{105}{\centi\meter} distance the average time was $0.76$ minutes and at \SI{210}{\centi\metre} the average time was $0.26$ minutes. The resolution of the thermal camera in the CAT S60 is $80\times60$, which seems to be sufficient for up to a meter. The thermometer scanner has a higher resolution $160 \times 120$, but a slower frame rate (\SI{6.67}{\hertz} vs. \SI{8}{\hertz}). For a \SI{210}{\centi\meter} distance, the thermometer fails to observe a proper thermal fingerprint. A higher resolution is thus not guaranteed to extend the operational range of \SystemName{} as also the frame rate needs to be considered.

%can be extended  increasing the resolution alone is unlikely to significantly extend the range of the imaging unless the frame rate of the of the camera can be increased. 

%However, with the thermometer scanner we were unable to observe a thermal fingerprint from  distance. This indicates that with the off-the-self thermal cameras, the maximum range to use our approach is about $1$ m, which is enough for equipping trash bins and transport recycling belts with our approach. This maximum range also is higher than the existing light reflectivity-based techniques. Notice that this limitation can be overcomed by using high resolution thermal cameras. However, this, in turn, increases the practical cost when using the approach.  



%\cparagraph{Temperature sensitivity} We also analyze whether slightly different temperatures influences the dissipation time of thermal fingerprints. To do this, we analyze further the BOTTLE material that was previously. induce a controlled temperature in the object, we rely on an incubator JANOEL18S with adjustable temperature. We put the object inside the incubator at a constant temperature for $15$ min to ensure that the entire object depicted the same temperature. We exposed the material to temperatures ranging from $36$\textcelsius~to $39$\textcelsius~degrees. We chose these temperatures as they depict normal and elevated temperature levels in a person. After the object was heated up, it was transferred to the tesed as depicted in Figure~\ref{fig:testbed}c and described in Section~\ref{sec:experimentalsetup}. We then proceed to measure the dissipation time of the thermal fingerprint. The room temperature that the object had to acclimatize range from $23$\textcelsius~to $23.5$\textcelsius~degrees. We obtained the next results of dissipation time for different temperature degrees (3.33 min for $36$\textcelsius~, 3.73 min for $37$\textcelsius~, 4.23 min for $38$\textcelsius~, and 4.34 min for $39$\textcelsius~ respectively). After the object was taken out from the incubator, its temperature dropped drastically from $36$\textcelsius~degrees to $33-32$\textcelsius~in a fraction of second. Nevertheless, the thermal fingerprints take different time periods to dissipate when exposed to different temperatures. Thus, our results indicate that small differences can be detected through thermal fingerprint analysis. While accurate human temperature is not possible to estimate, we envision that our approach can be used to detect abnormalities in human temperatures. For instance, in an airport, instead of monitoring the face of people with thermal cameras, it can be possible to monitor the tangible objects that people touch while passing security check. These could provide more insights on whether the person presents abnormal levels of temperature. 


\cparagraph{Temperature Sensitivity} We next analyze the sensitivity of the dissipation times to slight variations in temperature. 
%To enable other sophisticated use cases, e.g., abnormal human temperature, we also analyze whether slightly different temperatures influence the dissipation time of thermal fingerprints. To do this, 
To accomplish this, we further analyze the BOTTLE material in the fixed-hold condition, as above. We use a JANOEL18S incubator with adjustable temperature to achieve controlled changes in the temperature. We put the object inside the incubator at a constant temperature for $15$ min to ensure that the entire object has exactly the same temperature. We expose the material to temperatures ranging from \SIrange{36}{39}{\degreeCelsius}, corresponding to normal and elevated temperature levels in a human. After the object was heated up, it was transferred to the testbed that was used to record footage. We then proceed to measure the dissipation time of the thermal fingerprint. The room temperature that the object had to acclimatize ranges from \SIrange{23}{23.5}{\degreeCelsius}. The dissipation times for the different temperatures were: 3.33 min for \SI{36}{\degreeCelsius}, 3.73 min for \SI{37}{\degreeCelsius}, 4.23 min for \SI{38}{\degreeCelsius}, and 4.34 min for \SI{39}{\degreeCelsius} respectively. The dissipation time is expected to be a function of the temperature difference between the object and the environment, and our results confirm that these subtle temperature differences can be captured robustly using a commercial-off-the-shelf thermal camera. 
%After the object was taken out from the incubator, its temperature dropped drastically from \SI{36}{\degreeCelsius} to \SI{33}{\degreeCelsius} $-$ \SI{32}{\degreeCelsius} in a fraction of a second. Nevertheless, the thermal fingerprints take different time periods to dissipate when exposed to different temperatures. Thus, our results indicate that small differences can be detected through thermal fingerprint analysis. 
While accurate human temperature is not possible to estimate, we envision that our approach can be used to detect abnormalities in human temperatures. For instance, instead of monitoring the face of people with thermal cameras at an airport, it could be possible to detect abnormal temperatures by monitoring the tangible objects that people touch while passing a security check. %These could provide more insights into whether the person presents abnormal levels of temperature.



\subsection{Dissipation Time Classification Performance}
\label{ssec:classification}

We next demonstrate that our approach can support the coarse-grained classification of object materials based on the dissipation time of thermal fingerprints -- and other contextual factors. As described in Section~\ref{sec:methodology}, we considered three classification techniques: Random Forest (RF), Support Vector Machine (SVM), and Multi-Layer Perceptron (MLP). The results of the classification experiments are shown in Table~\ref{tab:classification}. When only the thermal fingerprint is available, the highest classification accuracy for material detection is approximately  $83$\%. %when only the dissipation time of the thermal fingerprint is available to predict the material type. 
Incorporating information about the hold pattern type does not improve the results, suggesting that the way people grasp the materials does not impact performance. 
%We can observe that Fixed-hold and Natural-hold are not informative parameters as the accuracy remains the same. 
In contrast, when having information about whether the person is male or female, we can observe that the accuracy to predict materials improves up to $86$\%. Similarly, when attempting to predict whether the user is male/female, we can observe that dissipation time and material information provide a high accuracy estimation of around $78$\%. %While not the focus of our work, this result has potential implications in interface and interaction design by offering information about the 

%is relevant for fostering the learning of autonomous systems based on interactions and personal characteristics of users. For instance, intelligent toys can change color based on female and male preferences. 

%Likewise, when predicting the contextual hold type and 



\begin{table}
\centering
\caption{Material classification accuracy (\%) in different experimental conditions. Model data $\rightarrow$ Predicted. Classification Method: Random Forest (RF), Support Vector Machine (SVM) and Multi-layer Perceptron (MLPC).}
\label{tab:classification}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Test} & \textbf{RF} & \textbf{SVM} & \textbf{MLPC} & \textbf{Average} \\
%\midrule
\hline %\Xhline{.8pt}
\textbf{Predicting Material (M)}
 &  &  &  \\
(Vector) $\rightarrow$M&90.9&77.3&81.8&\textbf{83.3}\\
(Vector, Context)$\rightarrow$M&90.9&77.3&81.8&\textbf{83.3}\\
(Vector, Gender)$\rightarrow$M&90.9&86.4&81.8&\textbf{86.4}\\
(Vector, Context, Gender)$\rightarrow$M&86.4&81.8&81.8&\textbf{83.3}\\
\quad\textit{Average}&\textit{89.8}&\textit{80.7}&\textit{81.8}&\textbf{\textit{84.1}}\\
\textbf{Predicting Context, Gender}
 &  &  &  \\
%\hline  
(Material, Vector)$\rightarrow$Context&77.3&81.8&72.7&\textbf{77.3}\\
(Material, Vector)$\rightarrow$Gender&77.3&77.3&81.8&\textbf{78.8}\\
\quad\textit{Average}&\textit{77.3}&\textit{79.6}&\textit{77.3}&\textbf{\textit{78.1}}\\

\bottomrule
\end{tabular}%
}
% \vspace{-.55cm}
\end{table}



\subsection{Comparison Against Other Approaches}

Next we compare \SystemName{} against the two baselines: computer vision and optical sensing. 
%We demonstrate that these techniques have limited discriminatory power in identifying material properties or objects in general. 
% Our main goal is to demonstrate that these approaches fail in identifying material properties and objects in general.
%first attempt to classify household objects using computer vision and 
We test  computer vision using 31 images depicting real tossed plastic objects~\cite{prata2020covid}. In total, 33 separate plastic items were present in the 31 images. The deep learning model managed to identify 23 of the 33 items (69.7\% in accuracy). \rev{Note that the goal is not to directly compare our approach against computer vision as they effectively address different problems. Indeed, the vision-based approach does not extract any internal characteristics of the objects and hence the only way it can be used in material recognition is to map specific item types to materials (e.g., drink bottles are typically made of PET). This approach works reasonably when the objects are sufficiently distinctive but fails in everyday use cases where the shape of the objects has changed, e.g., tossed objects often have lost their original shape, and other visual characteristics may similarly have undergone significant changes. Computer vision is also prone to occlusions and cases where the objects are only partially visible. These issues are highlighted in Figure~\ref{fig:baselines}a.  In practice computer vision and thermal dissipation can complement each other, e.g., autonomous ground vehicles could use computer vision to detect litter objects from afar, navigate next to the object, and use thermal dissipation to determine the material of the object. }

%Figure~\ref{fig:baselines} highlights the main limitation of the model, being unable to identify multiple objects simultaneously and objects whose shape changes drastically. 
%Although the trained model was primarily focused on plastics, such findings suggest that the application of using deep learning models and image vision for real life tossed object materials remains limited. 

\begin{figure}[!t]
\centering
    \begin{subfigure}[b]{.5\linewidth}
    \centering
    %\includegraphics[width=1.0\textwidth]{graphics/waste4.png}
    \includegraphics[width=0.8\textwidth]{graphics/fig9a.jpg}
   \caption{}\label{fig:baseline1}
   %fig:baselines
  \end{subfigure}   
  \begin{subfigure}[b]{.45\linewidth}
    \centering
    %\includegraphics[width=1.0\textwidth]{graphics/Material-reflection-laser.eps}
    \includegraphics[width=1.0\textwidth]{graphics/fig9b.png}
    \caption{}\label{fig:baseline2}
  \end{subfigure} 
  %\vspace{-15pt}
 % \caption{Baselines, a) Trained model PlasticNet, discriminating plastics against other object materials~\cite{prata2020covid}, b) Light reflectivity values of different materials measured with a photo-resistor.} 
  \caption{Baselines: (a) Trained model PlasticNet to identify and separate plastics from other object materials, and (b) Light reflectivity values of different materials measured with a photo-resistor.} 
  \label{fig:baselines}
  \vspace{-.4cm}
\end{figure}


Figure~\ref{fig:baselines}b shows the results for the second baseline, light reflectivity. %and compares them to two baseline backgrounds (white and black).
The low variation in reflectivity values indicates that light can accurately characterize different materials. However, we also observe  that different parts of the same material can be characterized very differently, e.g., Cardboard Cup-1 and Cardboard Cup-2. This is because objects comprise of different materials and colors, which can affect reflectance. Another limitation of this approach is the need for the sensors to contact the material to classify it accurately. 



\input{sections/Thickness}

==> The MIDAS Touch1/sections/Thickness.tex <==


\subsection{Effect of Thickness on Thermal Dissipation}
\label{ssec:thickness}

The results thus far have investigated the case where the camera can observe the objects that the user interacts with directly but in many practical scenarios the objects will be partially or fully occluded by other objects. \rev{We next demonstrate that thermal dissipation can be captured even in cases where the objects are covered by other objects. Naturally the thermal dissipation is affected by the materials that cover the object and hence the purpose of these experiments is to demonstrate the potential of our technique to support practical applications rather than to argue it can be used to detect materials through cover. }





\cparagraph{Experimental setup} Thermal radiation is absorbed from the outer side of an object material to its inner side as it dissipates. We conduct an experiment where thermal radiation from the outside of an object is absorbed and dissipated to its interior and used to model the thermal radiation of the object. As material influences thermal dissipation, as we have demonstrated previously, we design specialized samples to analyze the effect of thickness for thermal dissipation. These samples are developed from everyday household objects. In this experiment, we selected a plastic container (Plastic), a cardboard box (Cardboard), and a face mask (Mask) as baseline thickness for our samples (Figure~\ref{fig:thickness} shows the samples). We then aggregated multiple samples of the same object in layers to obtain samples with different thicknesses. \rev{Note that the overall penetration of the thermal radiation depends on two factors: (i) the thickness of the material and (ii) the characteristics of the material. These two factors together determine the thermal resistance of a material~\cite{mahlia2007correlation} which controls how much heat passes through, and thus also how much thermal radiation can be captured on the other side of the covering material.  In the experiments, we} consider a maximum of four layers as we found that thermal dissipation reduces significantly after this stage. The maximum thickness in the experiments is around \SI{2}{mm} which corresponds to the thickness of many everyday consumer products. For example, a plastic water bottle typically is between \SIrange{1}{2}{mm} thick. The material thickness in each layer is shown in Table~\ref{tab:tablethickness}. We rely on a Fujisan FJS025 electronic micrometer screw gauge having an accuracy of \SI{0.001}{mm} and range from \SIrange{0}{25}{mm} to measure the thickness of the objects. 


\begin{figure*}
	\centering
		\includegraphics[width=1.0\textwidth]{graphics/fig10.png}
	\caption{Thickness of object materials analyzed with thermal dissipation fingerprint.}
	\label{fig:thickness}
\end{figure*}



\cparagraph{Procedure} We measure thermal dissipation fingerprint from touch on the topmost material for one minute. After this, thermal dissipation is measured from the inner side of the object. This experiment is repeated three times per sample and multiple layers. We also measure the thermal dissipation time of the outer side of the object as a reference. The average body temperature of the human subject holding the object fell within \SIrange{36.4}{36.7}{\degreeCelsius}, and the ambient temperature was from \SIrange{22}{24}{\degreeCelsius}. Experiments were conducted for six days between 12:00 am and 14:00 pm.


\cparagraph{Results} Figure~\ref{fig:thickness1} shows the thermal dissipation estimated from the inner side of the object. The figure also includes the thermal dissipation fingerprint of objects from their outer side. From the results, we can observe \rev{two effects. First, the dissipation time increases as a result of larger surface area. Second, the dissipation time from the inside is smaller than the dissipation time from the outside with the total difference depending on the type and thickness of the material (i.e., higher thickness results in higher difference). Indeed, the difference is smaller for the plastic bottle compared with the face mask or the cardboard. This highlights how the effect of thickness depends also on the material that is covering the object. Nevertheless,} the results show that it is possible to observe that thermal radiation from human touch is visible even in samples with multiple layers. \rev{Besides demonstrating the robustness of the dissipation fingerprints against partial or full occlusion}, the result also has potential to support integration of \SystemName{} into everyday objects; see Section~\ref{sec:Discussion}.

%For all of the materials that were considered in the experiment, the maximal penetration is \SI{2}{mm}, i.e., at this point the material starts to serve as a resistance for thermal dissipation

%\textcolor{blue}{Figure~\ref{fig:thickness} shows the effect of thickness on thermal dissipation of materials like Plastic, Cardboard and Face Mask. We can see that the thermal dissipation time increases when the number of layers are increased. From the figure, we can also see the differences in thermal dissipation times from front Body side (Side from where the material was held and heat transfer took place) and Inner Body.}  

\begin{figure}[!t]
\centering
    \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig11a.png}
   \caption{One Layer Thickness}\label{fig:thicknesslayer1}
  \end{subfigure}   
  \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig11b.png}
    \caption{Two Layer Thickness}\label{fig:thicknesslayer2}
  \end{subfigure} 
  \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig11c.png}
    \caption{Three Layer Thickness}\label{fig:thicknesslayer3}
  \end{subfigure} 
  \begin{subfigure}[b]{.45\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/fig11d.png}
    \caption{Four Layer Thickness}\label{fig:thicknesslayer4}
  \end{subfigure} 
  %\caption{\textcolor{blue}{Effect on thermal dissipation with increase in the thickness of material} }
  \caption{Effect on thermal dissipation with increase in the thickness of material.}
  \label{fig:thickness1}
	   \vspace{-.4cm}
\end{figure}



\begin{table}[]
\centering
\caption{Material thickness in each layer for Cardboard, Plastic and Mask respectively.}
\label{tab:tablethickness}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
\textbf{Material Type}              & \textbf{Number of Layers} & \textbf{Thickness (mm)} \\ \hline
\multirow{4}{*}{\textbf{Cardboard}} & 1 layer                   & 2.801                   \\ \cline{2-3} 
                                    & 2 layers                  & 5.62                    \\ \cline{2-3} 
                                    & 3 layers                  & 9.183                   \\ \cline{2-3} 
                                    & 4 layers                  & 11.93                   \\ \hline
\multirow{4}{*}{\textbf{Plastic}}   & 1 layer                   & 0.44                    \\ \cline{2-3} 
                                    & 2 layers                  & 0.91                    \\ \cline{2-3} 
                                    & 3 layers                  & 1.53                    \\ \cline{2-3} 
                                    & 4 layers                  & 1.95                    \\ \hline
\multirow{4}{*}{\textbf{Mask}}      & 1 layer                   & 1.65                    \\ \cline{2-3} 
                                    & 2 layers                  & 3.23                    \\ \cline{2-3} 
                                    & 3 layers                  & 4.49                    \\ \cline{2-3} 
                                    & 4 layers                  & 6.13                    \\ \hline
\end{tabular}
}
\end{table}




%\cparagraph{Implications}
%\textcolor{blue}{We have shown \SystemName{} can identify the gender of an individual and can be seen on a thick body. With this in mind, Robot toys can respond or display emotions based on the individual who interacts with them. When a person touches the robot, the heat is transferred to the thermal sensor installed inside.}


==> The MIDAS Touch1/sections/UseCase.tex <==
\section{Detection of abnormal human temperature}

The previous sections demonstrated that human-emitted thermal radiation helps to characterize an object material from its surface and that the amount of thermal radiation absorbed by the object varies from individual to individual. We next demonstrate that our approach is not limited to supporting and optimizing waste management solutions, but can be used to enable novel and innovative sensing applications. As an example of such applications, we demonstrate how variations in dissipation time can be used to detect variations in human temperature. Direct monitoring of human temperature using thermal cameras is only feasible on expensive high resolution cameras that are taken from a specific region of the face~\cite{ring2012infrared}. Our approach overcomes these requirements by using indirect measurements obtained from thermal dissipation fingerprints. 

%being prominently differences between female and male hand-palms/finger-tips also exposed. Based on these findings, we next explore whether small changes in human temperature can be detected through the thermal fingerprint's dissipation time. The detection of elevated human temperature with thermal cameras is a challenging task, as it requires to take precise measurements from the small inner canthus/tear duct area in the face, which correlates the most with human temperature. Besides this, the thermal equipment required for the task is very costly (oscillating between $15,000 - 21,000$\$\footnote{https://www.midstateinstruments.com/flir-a320-tempscreen/}). Thus, to adopt the monitoring of human temperature with thermal cameras at a large-scale, new innovative approaches are required to apply thermal imaging technologies. Our approach can be adapted to overcome this gap, and we demonstrate this with controlled experiments.

\cparagraph{Experimental setup} We analyze further the BOTTLE material that we used in our previous experiments. To induce a controlled temperature in the object, we rely on an incubator JANOEL18S with adjustable temperature. We put the object inside the incubator at a constant temperature for $15$ min to ensure that the entire object depicted the same temperature. We exposed the material to temperatures ranging from $36$\textcelsius~to $39$\textcelsius~degrees. We chose these temperatures as they depict normal and elevated temperature levels in a person. After the object was heated up, it was transferred to the tesed as depicted in Figure~\ref{fig:testbed}c and described in Section~\ref{sec:experimentalsetup}. We then proceed to measure the dissipation time of the thermal fingerprint. The room temperature that the object had to acclimatize range from $23$\textcelsius~to $23.5$\textcelsius~degrees. We recorded video footage of the dissipation time using a CAT s60 smartphone. 


\cparagraph{Results} We obtained the next results of dissipation time for different temperature degrees (3.33 min for $36$\textcelsius~, 3.73 min for $37$\textcelsius~, 4.23 min for $38$\textcelsius~, and 4.34 min for $39$\textcelsius~ respectively). After the object was taken out from the incubator, its temperature dropped drastically from $36$\textcelsius~degrees to $33-32$\textcelsius~in a fraction of second. Nevertheless, the thermal fingerprints take different time periods to dissipate when exposed to different temperatures. In the figure, we can observe that dissipation time is shorter when  the temperature difference is smaller. The dissipation time increases as the temperature difference increases (takes $1.2$ min longer for temperature to fade when comparing $36$\textcelsius~against $39$\textcelsius~degrees). Our results indicate that small differences can be detected through thermal fingerprint analysis. While accurate human temperature is not possible to estimate, we envision that our approach can be used to detect abnormalities in human temperatures. For instance, in an airport, instead of monitoring the face of people with thermal cameras, it can be possible to monitor the tangible objects that people touch while passing security check. These could provide more insights on whether the person presents abnormal levels of temperature. 



% \begin{figure}
% 	\centering
% 		\includegraphics[width=0.7\columnwidth]{graphics/Abnormal-temperature-degrees.eps}
% 	\caption{Dissipation time of thermal fingerprints when exposed to different temperatures.}
% 	\label{fig:abnormal-temperature}
% \end{figure}




==> sections/Background.tex <==
\section{Background of study}
This section introduces public littering, which is considered a problem that plagues our society and the world. We also present background knowledge of the detection sensors, focusing on the thermal sensing technique and how it has been applied in computer systems. This technique is widely used in various fields of study. The thermal sensor can be integrated into an automated system such as autonomous robots or drones to detect common waste materials disposed on the streets, public areas, locate the material, and properly recycling it.  

\bparagraph{Public littering} Disposing of visible solid waste in wrong places or places they do not belong is considered as littering \cite{schultz2013littering}, \cite{campbell2007people}. It portrays a bad picture of the area, pollutes the environment, and costs a lot to clean up if not properly managed. Litter is distinct from other municipal solid waste (MSW) and includes any solid or liquid domestic debris. The most littered items are cigarette butts, takeout boxes, food wrappers, drink bottles or cans, broken glass, plastic bags. In 2007, the international coastal cleanup, Ocean Conservancy collected 6 million pounds of materials, which comprised of cigarette butts (27\% of the total number of items collected), bags(8\%), plastic beverage bottles (7\%), plastic utensils (5\%), caps and lids (9\%), and food wrappers (10\%) \cite{conservancy2007start}. Research has shown people's behavioural tendencies towards littering; there is a correlation between a littered environment and the intentional throwing of litter at that particular spot littered \cite{finnie1973field}. This means that when a place is littered, there is a higher propensity to experience increased littering. Littering is attributed to individuals as the primary source \cite{schultz2013littering}. 

Furthermore, it is estimated that 4.95 trillion cigarette butts are littered yearly worldwide, which also presents a threat to wildlife and, in some cases, fire outbreaks \cite{world2017tobacco}. Cigarette filters have been discovered in the stomachs of sea or marine creatures, birds who mistake them for food \cite{santos2005overseas}. Globally, different approaches have been adopted to curb littering to slow down climate change, such as providing the convenience of disposal facilities, public awareness on environmental education by promoting a positive attitude towards the environment, enforcement by handing out fines to perpetrators. There is no doubt that people have heard a lot about environmental problems, and they now want to hear a lot more about environmental solutions. 


\bparagraph{Passive sensing (IR Thermal imaging)}
According to J. Fraden,  “A sensor is a device that receives stimulus or an input signal and responds with an electrical signal bearing a known relationship to the input” \cite{fraden2003handbook}. Sensors can be found in most electrical devices and are designed for various applications, as well as aids surveillance, imaging, tracking, detecting, and mapping. Two categories of sensors consist of active sensor, which provides their source of light or illumination while also transmitting and detecting energy simultaneously. On the other hand, passive sensors do not provide illumination to produce output signals and measure variations based on natural emission \cite{brooker2009introduction}.

Infrared Thermal imaging, also known as Infrared thermography, is the recording and measurement of heat radiation. These are specially-designed cameras that work in an environment without any ambient light and can penetrate obscurants such as smoke, fog, and haze. The first Thermal cameras were originally developed for military purposes in 1950s and 1960s and have since evolved, enabling applications that were impossible to do easily in the past due to the high cost of production and limited availability. Thermal cameras are similar to digital photographic cameras but record thermal infrared radiation (TIR). Infrared radiation is invisible to the human eye as it occurs beyond the red end of the visible light spectrum (figure 1). However, thermal radiation is located within the infrared range of the electromagnetic spectrum \cite{kruse2001uncooled}. The visible wavelength range from $0.4 - 0.78\mu m$ while infrared radiation has a longer wavelength, ranging from $0.78-1000\mu m$ \cite{mehta2011introduction}; Thermal cameras operate in the infrared band of the electromagnetic spectrum with wavelengths between $2 - 14\mu m$. The infrared spectrum which is subdivided into near-infrared (NIR) $0.78 - 2.5\mu m$, mid-infrared (MIR) $1.3 - 8\mu m$ and far-infrared (FIR) $7.5\mu m$ and $13\mu m$ \cite{abdelrahman2017cognitive}, and are used for monitoring temperatures of different range from -50 to 2000$^{\circ}$C. All objects with a temperature above absolute zero (-273$^{\circ}$C) emit infrared radiation and not only objects we think of as warm emit infrared radiation (IR). Thermal imaging determines an image temperature based on the absolute temperature of the object. The image is formed base on the heat signature of the object and records current signatures of the objects based on their heat pattern.


%\begin{figure}
%	\centering
%		\includegraphics[width=0.4\textwidth]{graphics/spec.png}
%	\caption{The electromagnetic spectrum\cite{vadivambal2011applications}}
%	\label{fig:EngProto}
%\end{figure}

\subsection{Thermal detection types}
Thermal detection mechanism referred to as mechanism that change some measurable property of a material due to the temperature rise of that material caused by the absorption of electromagnetic radiation \cite{lloyd2013thermal}. Although there are several thermal detection mechanism, the most important are the resistive bolometric effect,  the pyroelectric effect and its modification known as either the biasenhanced pyroelectric effect or the ferroelectric bolometer, and the thermoelectric effect \cite{lloyd2013thermal}. Uncooled thermal detectors have been developed mainly with microbolometers thermal and ferroelectric detectors (uses Barium strontium titanate (BST) as detector material, which suffers from halo effect) \cite{gade2014thermal}. Microbolometers has the largest market share due to its advantages over ferroelectric detectors. 


\subsection{Application in computer systems}
With thermal imaging becoming popular, this section briefly discuses thermography as a useful technology in different fields. This detection technique is used in computer systems, which uses sophisticated image analysis algorithms and a computer to reconstruct the images to show heat patterns.

\bparagraph{Medical thermography} Computer systems are used for image processing and monitoring of thermal radiation changes. In medical analysis, thermography based computer-assisted detection/diagnosis (CAD) systems help to screen for fever patients in places with a high volume of people, such as airports and border crossings \cite{mercer2009fever}, \cite{sun2011portable}. The early detection of the diabetic foot,  specifically, CAD systems for diabetic foot \cite{adam2017computer}, help prevent complications and amputation. They have also been shown to reveal tumors in an early stage, most notably breast cancer \cite{qi2003thermal}. Medical issues such as the behaviour of ciliary muscle of the human eye \cite{harangi2011detecting}, the periodic fluctuation in skin temperature \cite{kondo2001thermal} or the measuring of blood flow rate in superficial veins \cite{mahmoud2013non}, can be studied from thermal images.

\bparagraph{Facial analysis} The face of an individual is a biometric trait that can be applied in an automated computer-based security system for authentication purposes. Experts are investigating and developing methods for the improvement of face recognition \cite{bhowmik2008classification}. Humans' stress level can be detected using thermal imaging, based on the heat radiation from their face. Thermal facial analysis was used for deception detection \cite{rajoub2014thermal}. Pavlidis et al. \cite{pavlidis2006detection} also propose this technique to capture anxiety. 

\bparagraph{Fire detection and military} With firefighters' inability to see through smoke quickly, they can be robbed of their most essential commodities (sight) when they fight fires and as such handicapping their ability to perform effectively, find the hot spot, and locate victims. Identification of objects that could pose a risk is of great importance. A fire detection system can be used for mobile robots \cite{hwang2010novel} by locating the hot spots, the robot is directed to the fire source. Arrue et al. \cite{arrue2000intelligent} proposed an alternative real-time infrared-visual system for forest fire detection, composed of both thermal and visual cameras, and meteorological and geographical information. In the military, Price et al. \cite{price2004system} presented the Gunfire Detection and Location (GDL) system for military applications to detect gunfire. Gunfire is detected in Mid-Wave IR (MWIR) imager and validated by acoustic events.










==> sections/Motivation.tex <==
\section{Motivation}
\label{sec:motivation}

\begin{figure}[!t]
\centering
    \begin{subfigure}[b]{.34\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/waste3.png}
   \caption{}\label{fig:waste1}
  \end{subfigure}   
  \begin{subfigure}[b]{.42\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{graphics/waste4}
    \caption{}\label{fig:waste2}
  \end{subfigure} 
  %\vspace{-15pt}
  \caption{Trained model PlasticNet, discriminating plastics against other object materials~\cite{prata2020covid}} 
  \label{fig:computer-vision}
\end{figure}



We begin by demonstrating how existing sensing techniques based on automated computer vision~\cite{white2020wastenet,ruiz2019automatic} and light sensing~\cite{singh2016iot} fail in identifying material properties and objects in general. \SystemName{} has been designed to overcome the limitations of these techniques by using material properties as the means for characterizing objects. 


\subsection{Computer vision analysis}

\cparagraph{Experiment} We first attempt to classify household objects using computer vision and train a state-of-the-art Convolutional Neural Networks (CNNs) model using the publicly available TrashNet dataset~\cite{aral2018classification}. We focus exclusively on the plastic materials category which contains $626$ images of plastic objects for training the deep learning model. Plastics are malleavable, so their accurate recognition is very sensitive to changes. The dataset has images where the individual pieces are shown against a white background. As such images do not match realistic recognition settings, we supplement the dataset with an additional $767$ images from the Japan Agency for Marine Earth Science and Technology (JAMSTEC) Deep-sea Debris Database dataset. %(additional 767 images).
%it was expected that such imagery would not match the real case of tossed and squashed waste against the background (e.g., pavement). For those reasons, we added 

Collected images were annotated manually by drawing a rectangle box around the object material in images. We labeled the TrashNet plastic items as "trash" and the JAMSTEC plastic items as "plastic". Both datasets were augmented by adding noise, hue, blue, horizontal flip, and vertical flip modifications to each original image, resulting in a total of 6985 for model training input. We created and trained the PlasticNet model using Google Collab server GPU, with 100k iterations and a batch size of 12, running TensorFlow Lite 1.15. For the base training model, ssd\_mobilenetv2\_oidv4 was used.

\cparagraph{Results} For validation, we used 31 images depicting real tossed plastic objects~\cite{prata2020covid}. In total, 33 separate plastic items were present in the 31 images. The deep learning model managed to identify 23 of the 33 items, obtaining 69.7\% in accuracy. Figure~ \ref{fig:computer-vision} highlights the main limitation of the model, being unable to identify multiple objects simultaneously and objects whose shape changes drastically. Although the trained model was primarily focused on plastics, such findings suggest that the application of using deep learning models and image vision for real life tossed object materials remains limited. 




\subsection{Light reflectivity analysis}
\cparagraph{Experiment} Reflectivity analysis of materials is a highly adopted technique to classify different material types~\cite{singh2016iot}. We next classify materials using light reflectivity measured through a photoresistor connected to the analog input pin of an Arduino MEGA ADK. The photoresistor captures light changes based on its resistance exposure to the light intensity of the reflected material. As a light source, we rely on a red laser diode (wavelength $650$ nm). The object was located $2$ cm away from the light source, depicting a practical usage of the sensor in transport belts and smart bins~\cite{white2020wastenet}. We took measurements with the sensor for different materials (selection described in Section~\ref{sec:materialselection}) during $1$ min from two different places of the object selected randomly. 

\cparagraph{Results} Figure~\ref{fig:Light-reflectivity} depicts the results and compares them to two baseline backgrounds (white and black). We can observe that light can characterize different materials with low variations, but that different parts of the same material can be characterized very differently, e.g., Cardboard Cup-1 and Cardboard Cup-2. This is because objects (end-products) consist of different materials and colors, both affecting its properties. A key limitation is that this approach requires a very short distance between the material and the sensor to classify the material accurately. Another limitation is that the light beam can cover a limited area, leaving most of the object untreated. 
 
\begin{figure}
	\centering
		\includegraphics[width=0.7\columnwidth]{graphics/Material-reflection-laser.eps}
	\vspace{-15pt}	
	\caption{Light reflectivity values of different materials measured with a photo-resistor.}
	\label{fig:Light-reflectivity}
\end{figure}

==> sections/UseCase.tex <==
\section{Detection of abnormal human temperature}

The previous sections demonstrated that human-emitted thermal radiation helps to characterize an object material from its surface and that the amount of thermal radiation absorbed by the object varies from individual to individual. We next demonstrate that our approach is not limited to supporting and optimizing waste management solutions, but can be used to enable novel and innovative sensing applications. As an example of such applications, we demonstrate how variations in dissipation time can be used to detect variations in human temperature. Direct monitoring of human temperature using thermal cameras is only feasible on expensive high resolution cameras that are taken from a specific region of the face~\cite{ring2012infrared}. Our approach overcomes these requirements by using indirect measurements obtained from thermal dissipation fingerprints. 

%being prominently differences between female and male hand-palms/finger-tips also exposed. Based on these findings, we next explore whether small changes in human temperature can be detected through the thermal fingerprint's dissipation time. The detection of elevated human temperature with thermal cameras is a challenging task, as it requires to take precise measurements from the small inner canthus/tear duct area in the face, which correlates the most with human temperature. Besides this, the thermal equipment required for the task is very costly (oscillating between $15,000 - 21,000$\$\footnote{https://www.midstateinstruments.com/flir-a320-tempscreen/}). Thus, to adopt the monitoring of human temperature with thermal cameras at a large-scale, new innovative approaches are required to apply thermal imaging technologies. Our approach can be adapted to overcome this gap, and we demonstrate this with controlled experiments.

\cparagraph{Experimental setup} We analyze further the BOTTLE material that we used in our previous experiments. To induce a controlled temperature in the object, we rely on an incubator JANOEL18S with adjustable temperature. We put the object inside the incubator at a constant temperature for $15$ min to ensure that the entire object depicted the same temperature. We exposed the material to temperatures ranging from $36$\textcelsius~to $39$\textcelsius~degrees. We chose these temperatures as they depict normal and elevated temperature levels in a person. After the object was heated up, it was transferred to the tesed as depicted in Figure~\ref{fig:testbed}c and described in Section~\ref{sec:experimentalsetup}. We then proceed to measure the dissipation time of the thermal fingerprint. The room temperature that the object had to acclimatize range from $23$\textcelsius~to $23.5$\textcelsius~degrees. We recorded video footage of the dissipation time using a CAT s60 smartphone. 


\cparagraph{Results} We obtained the next results of dissipation time for different temperature degrees (3.33 min for $36$\textcelsius~, 3.73 min for $37$\textcelsius~, 4.23 min for $38$\textcelsius~, and 4.34 min for $39$\textcelsius~ respectively). After the object was taken out from the incubator, its temperature dropped drastically from $36$\textcelsius~degrees to $33-32$\textcelsius~in a fraction of second. Nevertheless, the thermal fingerprints take different time periods to dissipate when exposed to different temperatures. In the figure, we can observe that dissipation time is shorter when  the temperature difference is smaller. The dissipation time increases as the temperature difference increases (takes $1.2$ min longer for temperature to fade when comparing $36$\textcelsius~against $39$\textcelsius~degrees). Our results indicate that small differences can be detected through thermal fingerprint analysis. While accurate human temperature is not possible to estimate, we envision that our approach can be used to detect abnormalities in human temperatures. For instance, in an airport, instead of monitoring the face of people with thermal cameras, it can be possible to monitor the tangible objects that people touch while passing security check. These could provide more insights on whether the person presents abnormal levels of temperature. 



% \begin{figure}
% 	\centering
% 		\includegraphics[width=0.7\columnwidth]{graphics/Abnormal-temperature-degrees.eps}
% 	\caption{Dissipation time of thermal fingerprints when exposed to different temperatures.}
% 	\label{fig:abnormal-temperature}
% \end{figure}



